Interactive Error Correcting Codes Over Binary Erasure Channels Resilient to $>\frac12$ Adversarial Corruption

An error correcting code ($\mathsf{ECC}$) allows a sender to send a message to a receiver such that even if a constant fraction of the communicated bits are corrupted, the receiver can still learn the message correctly. Due to their importance and fundamental nature, $\mathsf{ECC}$s have been extensively studied, one of the main goals being to maximize the fraction of errors that the $\mathsf{ECC}$ is resilient to. For adversarial erasure errors (over a binary channel) the maximal error resilience of an $\mathsf{ECC}$ is $\frac12$ of the communicated bits. In this work, we break this $\frac12$ barrier by introducing the notion of an interactive error correcting code ($\mathsf{iECC}$) and constructing an $\mathsf{iECC}$ that is resilient to adversarial erasure of $\frac35$ of the total communicated bits. We emphasize that the adversary can corrupt both the sending party and the receiving party, and that both parties' rounds contribute to the adversary's budget. We also prove an impossibility (upper) bound of $\frac23$ on the maximal resilience of any binary $\mathsf{iECC}$ to adversarial erasures. In the bit flip setting, we prove an impossibility bound of $\frac27$.

==> 3.5/explanation-temp.tex <==
\subsection{Protocol Overview}

Recall that in the  protocol resilient to $\frac6{11}$ erasures from \cref{sec:6/11}, Bob uses the codewords $\bar{0}$ and $\bar{1}$ to increment Alice's counter. Then, he wishes to ask a question about Alice's counter: either the \emph{value} of $x$ at index $\cnt$  or the \emph{parity} of $\cnt$. To do this, he sends one of two \emph{new} codewords $\bar{2}$ or $\bar{3}$. By including these two extra codewords, the maximal possible distance between Bob's possible codewords decreases from $1$ to $\frac23$, which incurs a loss in error resilience. When we increase this distance to $1$, it turns out that with the Alice to Bob message ratio of $4:1$ and $<\frac35$ erasures, there are many chunks in which both Alice's message is $2$-decodable and Bob's message is uniquely decodable, or Alice's message is uniquely decodable.

In this section, we show how to increment Alice's counter and ask a question \emph{without} the inclusion of these two additional codewords, which will increase the error resilience of the protocol to  $\frac35$ erasures.

In order to get rid of the need for the extra two codewords $\bar{2}$ and $\bar{3}$, we need for the two codewords $\bar{0}$ and $\bar{1}$ to be able to take on \emph{more than two meanings}. To do this, we combine our two codewords with \emph{timing cues}, such that $\bar{0}$ and $\bar{1}$ mean different things depending on where they are heard in the protocol. More specifically, we divide the protocol into \emph{blocks} of chunks, such that Alice interprets messages differently for the rest of the block depending on whether she first decoded a $\bar{0}$ or $\bar{1}$ within the block. The bits communicated in the rest of the block can now be combined with the first heard bit to take on more than two meanings. 

There are two pieces of information that Bob needs to convey, which he previously used the extra codewords for. These are:  
\begin{enumerate}
    \item Telling Alice she is done incrementing $\cnt$ (and thus can switch to answering Bob's question for the rest of the protocol). 
    \item Telling Alice which question (value or parity) to answer.
\end{enumerate}

First, we describe a new way to increment the counter via \emph{blocks}, which ultimately allows Bob to tell Alice to stop incrementing the counter without introducing a new codeword. Crucially, in this incrementation process, Alice always expects to hear $\bar{1}$ before $\bar{0}$ in every block, so she can reserve hearing $\bar{0}$ as the first message she hears in the block to mean that the incrementation is over. Then, we describe a second set of modifications to this protocol that specifies the question without introducing a new codeword.

\paragraph{Incrementation via blocks.}

Our new protocol is partitioned into many \emph{blocks}, which can be further divided into its many \emph{chunks} of rounds consisting of a single fixed-size message from each party in alternating order. There must be many (at least $\Omega(n)$) blocks with $<\frac35$ error, and in each of these, there will be many chunks with $<\frac35$ error. 

We now describe a new a different incrementation process that allows us to always begin blocks with $\bar{1}$.

At a high level, Alice tries to increment every block if the first bit she hears from Bob in that block is $\bar{1}$. However, since Bob defaults to starting blocks with $\bar{1}$, this would cause her to skip over $i$ sometimes, so instead she only increments if her last value of $\cnt$ is confirmed/acknowedged by Bob (which she tracks as $\sent$), which he tells Alice by sending $\bar{0}$ after his initial sequence of $\bar{1}$'s. Notice one problem: Bob cannot send Alice $\bar{0}$ in a block until he is \emph{sure} she has already received a $\bar{1}$. Therefore, when he is trying to confirm her value of counter, he still starts the block by sending $\bar{1}$, waits for Alice to tell him she has received a $\bar{1}$ in this block (for which we use a new boolean $\rec$ that she includes in her $\ECC$ denoting exactly this), and only then sends her $\bar{0}$. We outline the new protocol more precisely below.

\begin{itemize}
    \item 
        Every chunk, Alice sends her input $x$, along with a counter $\cnt$, a boolean $\sent$ detailing if her current value of $\cnt$ is confirmed, and a new $\rec$ which is $\true$ if she has received a $\bar{1}$ so far this block, encoded with a standard error correcting code.
    \item 
        At the start of every block, Bob sends $\bar{1}$'s.
    \item 
        When Alice receives a $\bar{1}$ in a block, she increments $\cnt$ if the previous value of $\cnt$ had been confirmed; otherwise, she does nothing.
    \item 
        If Bob learns that Alice has received a $\bar{1}$ this block, he attempts to confirm her value of $\cnt$ by sending $\bar{0}$ for the rest of the block. 
    
        If the two list-decoded versions of Alice disagree on whether $\bar{1}$ has been received, Bob sends $\bar{0}$ for the rest of the block anyway. This will make it possible for one of the two Alices to exit the incrementation stage early -- we show how to deal with this later.
    \item 
        If Alice gets Bob's $\bar{0}$, she confirms her new value of counter.
    \item 
        When Alice's value of $\cnt$ reaches $i$ or the counters differ, Bob sends $\bar{0}$ forever to indicate Alice should transitition.
    \item 
        If Alice hears $\bar{0}$ before ever hearing $\bar{1}$ in a block, she transitions out of the incrementation phase.
\end{itemize}

Like in the $6/11$ incrementation algorithm, Bob and Alice successfully increment while staying coordinated. However, we have the new property we wanted as well: \emph{Alice always receives $\bar{1}$ before $\bar{0}$ in each block}. Then, Bob starts a block with $\bar{0}$ to signal that the incrementation process is over (because the counters differ, or $i$ has been reached), and Alice should now transition to answering his question.
Now, if Alice could magically know which of the two questions she is supposed to answer, we would be done!

\paragraph{Specifying the question.}

Bob needs to tell Alice which question (\emph{value} or \emph{parity}) she needs to answer; if she could magically know the answer to this, we would be done, since she could send the singular bit that answers the question forever. We denote the stage where Alice is incrementing $\cnt$ as \emph{Stage 1}, and the stage where she is answering Bob's question as \emph{Stage 3}. 

Notice a couple things: if her answer to both questions are the same, she can immediately transition to Stage 3, without knowing what the question is. Moreover, we can get rid of the case where her answer to the \emph{parity} question is 1 and her answer to the \emph{value} question is 0 via the following trick. Instead of Bob's $i$ specificying the index of $x$ he wants, it specifies twice the index he wants. So if $\cnt$ is even, Alice's  answer to the \emph{value} question is actually $x[\cnt/2]$. Bob will never choose $i$ to be odd, so if Alice were to finish incrementation of $\cnt$ at an odd counter, she can be confident Bob wants an answer to the parity question, and thus send $1$'s forever. 

As such, the only case where Alice actually needs to learn what question to answer is where her \emph{parity} bit is $0$ and her \emph{value} bit is $1$. In this case, when Alice receives the go ahead to transition, she will transition to \emph{Stage 2} instead of Stage 3. In Stage 2, she tries to learn what Bob's question is, assuming her answers to \emph{value} and \emph{parity} are $1$ and $0$ respectively.

It may be tempting for Bob to simply send $\bar{0}$ to indicate one question, and $\bar{1}$ to denote the other -- however, how does Alice distinguish this $\bar{0}$ that specifies this question from the $\bar{0}$ that transitioned her to Stage 2? Maybe Bob just hasn't yet noticed her transition. Therefore, we must use a more complicated procedure: when Bob detects one version of Alice is in Stage 2, he and Alice increment a second counter, denoted $\knt$. When Alice receives the signal to transition again (i.e. the first message received in a block is $\bar{0}$), the value of $\knt \in \{ 0, 1 \}$ tells her which question Bob wants answered. This counter increments the same way as $\cnt$, and Alice reuses the booleans $\sent$ and $\rec$ to assist with this incrementation. Throughout the protocol, she sends Bob $\knt$ as part of her $\ECC$ to tell him what the value is at any given time (it will be $-1$ initially). Then, when it reaches the desired value, Bob will transition Alice out of Stage 2 by sending $\bar{0}$ at the start of the block.

However, it is important that Bob's attempts to increment $\knt$ for one version of Alice do not interfere with what he is doing for the other version of Alice. We deal with this separately based on what case the other Alice is in. If it is in Stage 3, Bob can freely direct all his efforts to incrementing and transitioning the Stage 2 Alice; the Stage 3 Alice ignores him forever. The other Alice cannot be in Stage 2, as the two versions of Alice cannot advance with the same answer to both \emph{value} and \emph{parity} questions by design. 

Finally, we reach the difficult case where the other Alice is in Stage 1. If Bob tries to simultaneously increment both counters simultaneously and then transition both simultaneously, as he would if both were in Stage 1, he cannot necessarily coordinate them to send opposite bits forever -- since the Alice in Stage 1 can really be anywhere in her $\cnt$ incrementation, so the value she would answer simultaneously incrementing $1$ or $2$ times with Bob could be anything. To solve this problem, we have certain points at which Alice's counter value is reset back to 0. We introduce a final layer of round grouping: the \emph{megablock}. That is, our final protocol consists of many \emph{megablocks}, each containing many blocks, which each consist of many chunks, each made up of a single many-round message from Alice followed by a many-round message from Bob. At the beginning of each megablock, Alice resets the counter she is currently incrementing (either $\cnt$ or $\knt$) to $0$. In other words, she returns to the beginning of the stage she is currently in.

Then, it turns out if Bob knows at the beginning of a megablock that one version of Alice is in Stage 1 and the other is in Stage 2, he can just send $\bar{0}$ forever! The one in Stage 1 eventually transitions with $\cnt=0$ which we define to correspond to transitioning to Stage 3 with the bit $0$. The one in Stage 2 eventually transitions with $\knt=0$ which we know answers the \emph{value} question, which must have answer $1$.

It requires a bit of effort to understand why these new megablocks do not interfere with any of the protocol design thus far, but the idea is that resetting the process only slows Alice and Bob down; it doesn't confuse Alice any more about Alice's state (since he knows exactly when she will reset and what she will reset to).

% Bob needs to tell Alice which question (\emph{value} or \emph{parity}) she needs to answer. To do this, he and Alice increment a second counter, denoted $\knt$. When Alice receives the signal to transition again (i.e. the first message received in a block is $\bar{0}$), the value of $\knt \in \{ 0, 1 \}$ tells her which question Bob wants answered. In detail, Alice begins the protocol in \emph{Stage 1}, in which she increments $\cnt$. When she first hears a $\bar{0}$ at the beginning of a block, she advances to \emph{Stage 2} in which she now increments $\knt$ the same way she had been incrementing $\cnt$. When she hears a $\bar{0}$ first in a block again, she determines Bob's question as \emph{value} if $\knt = 0$ and \emph{parity} if $\knt = 1$, and advances to \emph{Stage 3}. In Stage 3, she sends the bit answer to that question repeatedly for the rest of the protocol.

% There are a couple shortcuts:  \ynote{These shortcuts are to achieve a better error resilience parameter?} if her answer to both questions are the same, she can bypass Stage 2 and advance immediately to Stage 3. Moreover, we can get rid of the case where her answer to the \emph{parity} question is 1 and her answer to the \emph{value} question is 0 via the following trick. Instead of Bob's $i$ specificying the index of $x$ he wants, it specifies twice the index he wants. So if $\cnt$ is even, Alice's  answer to the \emph{value} question is actually $x[\cnt/2]$. Bob will never choose $i$ to be odd, so if Alice were to finish incrementation of $\cnt$ at an odd counter, she can be confident Bob wants an answer to the parity question, and thus send $1$'s forever. As such, the only case where Alice still needs to learn what question to answer is where her \emph{parity} bit is $0$ and her \emph{value} bit is $1$, and only in this case does she actually advance to Stage 2.

% One has to take care and make sure that Bob can coordinate the two worlds to end up in Stage 3 answering different bits. To do this, it is helpful to have certain points at which Alice's counter value is reset back to 0. We introduce a final layer of round grouping: the \emph{megablock}. That is, our final protocol consists of many \emph{megablocks}, each containing many blocks, which each consist of many chunks, each made up of a single many-round message from Alice followed by a many-round message from Bob. At the beginning of each megablock, Alice resets the counter she is currently incrementing (either $\cnt$ or $\knt$) to $0$.  

\paragraph{Final protocol.}

The final protocol is as follows. We assume that whenever Bob list-decodes Alice's message to 2 states that both states are consistent with previous pairs of states, that is, they are possible values of Alice's current state if she had been in the previous state and had seen some subset of Bob's message since the last 2-decoding. Otherwise, if Bob list-decodes to states such that only one is consistent with a past state, he learns $x$ and doesn't need to go through with the rest of the protocol.

\begin{enumerate}
    
    \item Alice and Bob begin by following the protocol from the previous section to increment $\cnt$ in each megablock. At the start of each megablock, Alice resets $\cnt$, and Bob, knowing this, restarts the incrementation. 
    %This phase, where Bob sees that both Alices are still in Stage 1, is \emph{Phase 1}.
    
    % \item If $\cnt_0 = \cnt_1$ ever reaches the index $i$, or $\cnt_0 \not= \cnt_1$, Bob switches to sending $\bar{0}$ continuously, ignoring all block barriers. He does this until he hears that at least one Alice has advanced to Stage 2 or 3, at which point he switches to sending $\bar{1}$'s for the rest of the megablock. \rnote{did we agree that this happens? i sorta forget why but i remember talking about it}
    
    % It's also possible that Alice advances to Stage 2 or 3 without Bob having switched to sending $\bar{0}$ continuously (Bob sends $\bar{0}$ for the rest of the block in the case that he sees that one Alice has received a $\bar{1}$ and the other has not). If Bob sees that this happens, he sends $\bar{1}$ for the rest of the megablock.
    
    \item Eventually, one of two things will happen.
    
    \begin{itemize}
        \item Bob begins sending $\bar{0}$'s for the rest of the megablock to tell both Alices to advance from Stage 1 to Stage 2 or 3. 
        
        \item At some premature point, before the conditions for asking both Alices to advance have been reached, Bob sees that exactly one of the Alices has already advanced. This is possible if at some point Bob sees that one Alice has received a $\bar{1}$ while the other has not, since in that case he sends $\bar{0}$ for the rest of the block.
    
        % \item Bob encounters a point where exactly one Alice has received a $\bar{1}$ and the other has not. Then, he sends $\bar{0}$ for the rest of the block to tell only that one Alice to advance from Stage 1 to Stage 2 or 3.
    \end{itemize}
    
    % It's also possible (since Bob sends $\bar{0}$'s for the rest of the block if he sees that one Alice has received a $\bar{1}$ and the other has not) that at some premature point exactly one of the two Alices advances to Stage 2 or 3, while the other stays in Stage 1. 
    
    \item Alice advances to Stage 2 (and possibly auto-advances to Stage 3) if the first message she receives in a block is a $\bar{0}$. In stage 2, starting with the next megablock after first advancing to Stage 2, Alice increments $\knt$ instead of $\cnt$, resets $\knt$ (and not $\cnt$) at the start of every megablock, and advances to Stage 3 when she hears $\bar{0}$ at the start of a block.
    
    \item When Bob sees that at least one Alice has advanced to Stage 2 or 3, he sends $\bar{1}$'s for the rest of the megablock, and changes his strategy in the next megablock. Note that both versions of Alice cannot be in Stage 2, since then they would both have $\cnt ~\text{mod}~ 2 =0$ and $x[\cnt/2] = 1$, but Bob only allows both Alices to advance if the two Alice's have different values of $\cnt~\text{mod}~2$ or $x[\cnt/2]$. 
    %to \emph{Phase 2} or \emph{Phase 3} at the beginning of the next megablock depending on if the two Alices are in Stage 1 and 2, or at least one is in Stage 3, respectively. We note that it is not possible for both Alices to have advanced to Stage 2, since the only way both Alices can advance is if Bob sees that their states are off by one in some way: either their counters are 1 apart or the values of $x[\cnt/2]$ are different. It is impossible for both Alices to advance and also both have even $\cnt$ and $x[\cnt/2] = 1$.
    
    \begin{caseof}
        \case {One Alice is in Stage 1, and the other is in Stage 2.} 
            {It is the beginning of the megablock so the Alice in Stage 1 has $\cnt = 0$ and the Alice in Stage 2 has $\knt = 0$. Bob simply sends $\bar{0}$ for the rest of the protocol, so that when the Alices advance to Stage 3, they do so with opposite bits: the Alice in Stage $1$ answers $0$, and the Alice in Stage $2$ answers $x[\cnt/2] = 1$.}
        \case {One Alice is in Stage 1 or 2, and the other Alice is in Stage 3.} 
            %If both Alices are in Stage 3, they've advanced here with opposite bits, since they may both advance only when Bob asks them to when he sees either $\cnt_0 \not= \cnt_1$ or $x_0[\cnt_0/2] \not= x_1[\cnt_1/2]$.
            %Otherwise, if exactly one Alice is in Stage 3 and the other is in Stage 1 or 2
            {The answer $b \in \{ 0, 1 \}$ of the Stage 3 Alice is fixed, so Bob can focus on incrementing the remaining Alice's counter to a value for which her answer to Bob's question is $1-b$.}
    \end{caseof}
    
    \item At the end of the protocol, Bob should have coordinated both versions of Alice to send opposite bits forever; hearing any one bit from Alice now suffices to deduce $x$.
    
     
    
    % \item Bob will begin the next megablock by sending $\bar{1}$. The first time he hears a message from Alice, if both versions of Alice are still on Stage 1, he goes back to Step 1, and re-does it. If at least one version of Alice advanced, he sends $\bar{1}$ for the rest of the megablock, and moves to the next step at the start of the next megablock.
    % \item Bob acts differently in each of the following cases for the two versions of Alice.
    % \begin{caseof}
    %     \case {Both versions of Alice are in Stage 3.} {They must have had opposite answers for both questions, so Bob can use a single bit from Alice to deduce $x$ as desired.}
    %     \case {Exactly 1 version of Alice is in Stage 3.} {That version is sending bit $b$ forever (Bob knows $b$). The other version of Alice is in Stage 1 or 2; Bob can increment $\cnt$ or $\knt$ until Alice's answer to the final question will be $(1-b)$.}
    %     \case {One version of Alice is in Stage 1 and the other in Stage 2.} {This is where it is important that we reset $\cnt$ -- Bob can just send $\bar{0}$ forever, since we can impose that advancing when $\cnt=0$ directly takes Alice to sending $\bar{0}$ forever. The version of Alice in Stage 2 will conclude $\knt=0$ and send $\bar{1}$ forever.}
    %     \case {Both versions of Alice are in Stage 2.} {This cannot happen, because then both \emph{parity} and \emph{value} questions have the same answer, and Bob never advances Alice when that holds.}
    % \item At the end of the protocol, Bob should have coordinated both versions of Alice to send the opposite bits forever; hearing any one bit from Alice now suffices to deduce $x$.
    % \end{caseof}
\end{enumerate}

\noindent We provide the formal protocol in the next section.

\rnote{todo: mention what $\stg$ is}

==> 3.5/old-explanation.tex <==
Recall that in the $\frac6{11}$ protocol from the previous section, Bob uses the codewords $\bar{0}$ and $\bar{1}$ to increment Alice's counter. Then, when he wishes to ask a question about Alice's counter (either the value of $x$ at index $c$ or the parity of $c$), he has to send one of two \emph{new} codewords $\bar{2}$ or $\bar{3}$. By including these two extra codewords, the maximal possible distance between Bob's possible codewords decreases from $1$ to $\frac23$, and we get a loss in erasure resilience. In this section, we show how to increment Alice's counter and ask a question \emph{without} the inclusion of these two additional codewords.

The main idea is to replace the two extra codewords with \emph{timing cues}. In particular, we note that $\bar{0}$ and $\bar{1}$ can mean different things according to the relative order they are heard in regards to absolute timing markers. For instance, if there are timing markers at rounds $k_1 < k_2$, whether Alice hears a $0$ or a $1$ first between these two rounds can mean very different things. Furthermore, hearing a $1$, followed by hearing a $0$, can mean something different than just hearing a $1$.

We have to be careful, though, since if hearing a relative sequence of $1, 0$ means something drastically different than simply hearing a $1$, a clever adversary will let Alice hear the first $1$, and then erase all of Bob's future messages so that she cannot distinguish whether Bob had intended to send $1,0$ or just $1$. In our case, if Alice hears just a $1$ between two timing markers, progress is simply delayed: she expects to hear a $1$ between the next set of timing markers and does not move on until she hears also a $0$. This strategy (delay until Alice hears a $1$ followed by a $0$) is reminiscent of the incrementation strategy from the $6/11$ protocol (delay incrementation until Alice hears a new value of $\bar{0}$ or $\bar{1}$): indeed, in our new protocol, incrementation is achieved by the single message pattern $1,0$ between timing markers rather than by two different message patterns (switching from $1$ to $0$ or vice versa).

This leaves sending $\bar{0}$'s exclusively between two timing markers available for a separate meaning. In our protocol, we delegate this message pattern to mean that Bob is done incrementing and wishes for Alice to answer a question.

There are several more design choices needed to make this idea work. We discuss these choices in Section~\ref{sec:3/5-high-level}, and leave a detailed description of the protocol and its formal analysis to Sections~\ref{sec:3/5-formal} and~\ref{sec:3/5-analysis}.

\subsection{Protocol Overview} \label{sec:3/5-high-level}

Let us start by describing the incrementation strategy in more detail.

\paragraph{Incrementation via blocks.}

Consider a protocol partitioned into many \emph{blocks}, which can be further divided into many \emph{chunks} of rounds consisting of a single fixed-size message from each party in alternating order. In each block, there is a chance for Bob to increment Alice's counter by $1$ by sending her $\bar{1}$'s followed by a $\bar{0}$'s so that Alice is guaranteed to see a $1$ before seeing any $0$'s. If Alice's current value of counter is confirmed (denoted by $\sent = \true$), she increments her counter the first time in a block she sees a $1$ from Bob. Then, when she sees a $0$, she marks the incrementation as confirmed (i.e. sets $\sent = \true$). If she only sees $1$'s in a block, her current counter value is unconfirmed and she does not further increment until it has been confirmed in a future block by receiving a $0$ after receiving a $1$. If the first bit Alice sees within a block is a $0$, she \emph{advances}: the incrementation stage is over. For now, we think of her advancement as to a permanent, question answering phase (that is, she sends the same message each chunk for the rest of the protocol, regardless of what she receives from Bob).

On Bob's end, when he wishes to increment or confirm Alice's counter, he begins a block by sending $\bar{1}$'s. If Alice receives any of his $1$'s, he wishes to send $\bar{0}$'s for the rest of the block, so that she knows that he's confirmed the incrementation. But he can only send $\bar{0}$'s once he \emph{knows for sure} that she's seen a $1$ and incremented her counter, otherwise Alice may first see a $0$ and interpret Bob's message as an \emph{advance request}.

To solve this, Alice keeps track of a boolean value $\rec \in \{ \true, \false \}$ that tells whether she has received a $1$ so far this block, and each chunk sends $\rec$ in addition to $x$ and $\cnt$ to Bob. Then, when Alice has received a $1$ and is ready to receives $0$'s, Bob can tell by decoding her message and reading the value of $\rec$.

In the $6/11$ protocol, the moment Bob list decodes to 2 possible worlds in which either the counters are different or both counters are equal to the index $i$, he begins sending $\bar{2}$'s or $\bar{3}$'s to ask Alice a question. This becomes more complicated with blocks, as Bob cannot formally start asking a question until the start of the next block. Furthermore, with the new variable $\rec$, we must take care in specifying Bob's behavior for the various pairs of values of $\cnt, \rec$, since Bob can no longer simply ask a question whenever $(\cnt_0, \rec_0) \not= (\cnt_1, \rec_1)$. In what follows, we do some case studies and describe Bob's behavior in each.
\begin{itemize}
    \item 
        If each time Bob decodes Alice's message to 2 states the values of $\cnt$, $\sent$, and $\rec$ are always the same, then Bob's job is easy: he can simply act as if he is incrementing one of them. That is, in each block he sends $\bar{1}$'s until he sees that $\rec_0 = \rec_1 = \true$, then he sends $\bar{0}$'s. More specifically, 
        \begin{itemize}
            \item If $\rec_0 = \rec_1 = \false$, Alice has not seen any $1$'s this block, and Bob continues sending $\bar{1}$'s.
            \item If $\rec_0 = \rec_1 = \true$ and $\sent_0 = \sent_1 = \false$, Alice's counter is in need of confirmation and she's already seen a $1$ this block, so Bob sends $\bar{0}$'s.
        \end{itemize}
        The case $\rec_0 = \rec_1 = \true$ and $\sent_0 = \sent_1 = \true$ should never occur, as $\rec = \true$ implies an unconfirmed bit while $\sent = \true$ implies a confirmed bit.
    \item 
        If ever Bob decodes to 2 states in which $\cnt_0 \not= \cnt_1$, ideally Bob would begin asking a question immediately. However, he may not be able to do so until the next block, since Alice may have already seen a $1$ this block. Bob also needs to prevent Alice from incrementing any more, otherwise it's possible that by the end of the block the two values of $\cnt$ are once again equal and Bob's question would be fruitless. Thus, Bob begins sending $\bar{0}$'s immediately. This at most confirms the larger of $\cnt_0, \cnt_1$, and stops the smaller from incrementing. Note that the world corresponding to the smaller $\cnt$ may advance that block, but as the (unequal) value of $\cnt$ is preserved in either case this presents no issues.
    \item 
        Consider the case where Bob is sending $\bar{0}$'s to confirm a bit, and one world notes the $0$ and marks $\sent = \true$, while the other does not. Then, at the beginning of the next block, $\cnt_0 = \cnt_1$ and $\rec_0 = \rec_1 = \false$, but (w.l.o.g.) $\sent_0 = \false$ but $\sent_1 = \true$. 
        
        Bob begins the block by sending $\bar{1}$'s. Note that if the world corresponding to $x_1$ sees a $1$, it will further increment $\cnt_1$. Meanwhile, even if the world corresponding to $x_0$ sees a $1$, it cannot increment $\cnt_0$ since $\sent_0 = \false$. Then, the next time Bob is able to 2-decode he will see that $\cnt_0 \not= \cnt_1$! 
        
        However, it's also possible that the world corresponding to $x_1$ doesn't see a $1$, while the world corresponding to $x_0$ does. Then, the two worlds are $(x_0, \cnt_0, \sent_0 = \false, \rec_0 = \true)$ and $(x_1, \cnt_1, \sent_0 = \true, \rec_0 = \false)$, where $\cnt_0 = \cnt_1$. Here, the problem with Bob continuing to send $\bar{1}$'s is that if the state corresponding to $x_0$ were Alice's true state, then the adversary could artificially confuse Bob with a state with $\sent_0 = \true$ and $\rec_0 = \false$, such that Alice can receive every message from Bob in its entirety but yet no progress can be made! Instead, in this case Bob switches to sending $\bar{0}$'s for the rest of the block. The state corresponding to $x_0$ may at most confirm $\cnt_0$. Meanwhile, it's possible that the state corresponding to $x_1$ advances. If this happens, the next time Bob 2-decodes, one state will have advanced, and the other state has incremented $\cnt_0$ at most once more (note that Bob only sends $\bar{1}$'s until he is able to $2$-decode). Since advancing is nonreversible, Bob is left with a single state still in the original incrementation phase. He can now focus on incrementing the remaining counter $\cnt_0$ until it reaches a value for which Alice's answer for state $0$ differs from her answer for state $1$.\footnote{As we will discuss in a bit, our final protocol uses \emph{megablocks}, which are groups of blocks. Instead of Bob trying to further increment $\cnt_0$ immediately, in our protocol will actually have Bob wait until the beginning of the next megablock to begin the incrementation process again.}
        % Bob prevents any more updates by sending $\bar{1}$'s for the rest of the megablock, and in the next megablock increments $\cnt_0$ (which is reset to $0$) until it reaches a value for which the answer for state $0$ differs from the answer for state $1$.
    \item 
        There's also the possibility that $\sent = \false$ in both worlds, yet one world has seen a $1$ ($\rec = \true$) and the other has not ($\rec = \false$). As in the previous situation, Bob sending $\bar{1}$'s here permits an adversarial attack that halts all progress for no corruption price. Thus, here, too, Bob begins sending $\bar{0}$'s. If neither world sees any $0$'s, then up to the first time Bob 2-decodes in a future block, both states will still be the same, except with possibly different values of $\rec$. Although no progress was made, this cost the adversary a good fraction of budget no matter which world Alice was in. Otherwise, if the world corresponding to $\rec = \false$ sees a $0$, it will advance. In this case, similar to the above case, once Bob 2-decodes and notes the advance, he focuses on incrementing the remaining $\cnt$ until it reaches an appropriate value. 
        
        The final case is if the world corresponding to $\rec = \true$ sees a $0$ but the world with $\rec = \false$ does not. Then, the world with $\rec = \true$ confirms the value of $\cnt$ (sets $\sent = \true$). Then at the beginning of the next block, the two worlds will have the same value of $\cnt$ but different values of $\sent$. In particular, the next time Bob successfully 2-decodes and one of the states has seen a $1$, either $\cnt_0 \not= \cnt_1$, or $\cnt_0 = \cnt_1$ but (w.l.o.g.) $(\sent_0, \rec_0) = (\true, \false)$ and $(\sent_1, \rec_1) = (\false, \true)$. All in all, this case cannot loop for no cost.
        \rnote{i think this is all the cases....?}
\end{itemize}

\paragraph{Specifying the question.}

Thus far, when Alice advances, we assumed she goes straight to answering Bob's question. However, how does she know what the question is? From her point of view, she only knows the value of her counter and the fact that Bob wished for her to advance, but she cannot distinguish whether the question was for the $\cnt$'th bit of $x$ or the parity of $\cnt$. We will call these \emph{value} and \emph{parity} questions for short. Without gaining more information about Bob's question, Alice has to answer both questions, for a total of $4$ possible responses. 

We can reduce this to $3$ possible responses via the following trick:  if $\cnt$ is even, Alice answers with the bit of $x[\cnt]$. Otherwise she replies with a third word indicating that the parity of $\cnt$ is odd. That is, only even values of $\cnt$ refer to actual indices.

In order to further reduce the number of possible responses to $2$, Bob will need to specify his question. Note that out of the previous set of 3 responses, two of them have a fixed answer $\in \{ 0, 1 \}$ no matter which question Bob asks: if $\cnt$ is even and $x[\cnt] = 0$, Alice answers $0$ in either case, and if $\cnt$ is odd, the only valid question Bob may ask is the parity of $\cnt$, to which Alice responds $1$. The final response is ambiguous, as Alice could answer $1$ if Bob asked for the value and $0$ if Bob asked for the parity.

If Alice is in one of the first two cases, she doesn't need further specification to be able to answer Bob's question, so she can go directly to the answering stage and begin answering it. Thus, when she advances, she immediately begins sending all $0$'s or all $1$'s to indicate what her answer to Bob's question must be. In the third case, $\cnt = 0~\text{mod}~2$ and $x[\cnt/2] = 1$, she goes to a different stage, where Bob will provide her with more instruction.

In this new stage, Bob increments a \emph{second} counter to convey to Alice which question he wants answered. We denote the value of this counter by $\knt$. $\knt$ begins at $0$ at the beginning of the stage, and is incremented in the same way as $\cnt$ was. When Alice advances from this stage to the answering stage with a value of $\knt$, she determines Bob's question as value if $k = 0$ and parity if $k = 1$. She then sends the bit answer to that question repeatedly for the rest of the protocol.

If one of the two list-decoded states is already in the answering stage, that world will disregard all future messages from Bob, so Bob's task of incrementing the remaining counter (either $\cnt$ or $\knt$) is straightforward. However, it is possible for one world to still be incrementing $\cnt$, while the other is in the $\knt$ incrementation stage. We have to guarantee that Alice's final answers in the two worlds are distinct.

It is not immediately obvious how to do this. If $\cnt$ and $\knt$ increment at the same rate, Bob's task is simple, but if one increments and the other doesn't, Bob can't just ask Alice for the parity of her counter. To solve this problem, we note that if we could reset both $\cnt$ and $\knt$ to their initial values of $0$, then Bob can send $\bar{0}$'s immediately to ask Alice to advance without incrementing, such that her answers in the two cases are determined and \emph{distinct}. That is, if she holds $\cnt = 0$, Alice sends $0$'s as her final answer (note that $\cnt/2 = 0$ is not a valid index, so we artificially prescribe this behavior), and if she holds $\knt = 0$, she sends the value of $x[\cnt/2]$, which must've been $1$ for her to end up in this stage at all!

\paragraph{Megablocks.}

In order to allow the resetting of the counters, we introduce a final layer of round grouping: the megablock. That is, our final protocol consists of many \emph{megablocks}, each containing many \emph{blocks}, which each consist of many \emph{chunks}, where a chunk is a single many-round \emph{message} from Alice followed by a many-round message from Bob. At the beginning of each megablock, Alice resets her counter (either $\cnt$ or $\knt$ depending on which stage she is in). Then, within the megablock, Bob increments her counter via the blocking strategy we've discussed, and if the incrementation is successful (or the two counters become misaligned), he sends her advance requests consisting of $\bar{0}$'s. If Alice receives an advance request, she advances either directly to the answering phase, or to the $\knt$ incrementation phase (if she is not already incrementing $\knt$). 

One final detail is how Bob learns what stage Alice is in. For instance, he may be sending advance requests at the end of a megablock, but if he can never 2-decode Alice's messages he may not learn during that megablock if either world has advanced. Instead, we leave the deduction of Alice's current stage to the next megablock. That is, Bob can learn the two Alice stages the first time in the next megablock he $2$-decodes Alice's message.

==> 3.5/old-lemma4.3.tex <==

\begin{lemma} \label{lem:megablock-budget}
    Suppose that Bob never decodes Alice's message to exactly 1 state, and that every time Bob $\le 2$-decodes Alice's message, the resulting pair of states is consistent with previous pairs. Assume that at the beginning of a megablock $(s_0, s_1) \not= (3, 3)$, and also that Alice's true input is $x_b$ such that $s_b < 3$. If at the end of the megablock the value of $(s_0, s_1)$ has not changed, then at least $\frac35 - \frac{12}{5}\epsilon$ of the rounds in that megablock were corrupted.
\end{lemma}

\begin{proof}
    First note that if either world had advanced since the last $2$-decoding prior to the start of the megablock (i.e. when $\st_0, \st_1$ were set), then if Bob $2$-decodes any message this megablock, the value of $(s_0, s_1)$ will have changed by the end of the megablock. In this case, the adversary must erase at least $\frac34 - \frac32\epsilon$ of each of Alice's messages, for a total erasure rate of $\frac{(\frac34 - \frac32\epsilon) \cdot 4M}{5M} = \frac35 - \frac65\epsilon$.
    
    Otherwise, suppose that neither world has advanced since the setting of $\st_0, \st_1$, so that the two worlds are in Stages $s_0$ and $s_1$ respectively the beginning of the megablock. We will proceed by cases over the possible values of $(s_0, s_1) \not= (3, 3)$ at the beginning of the megablock.
    \begin{caseof}
        \case{$s_0 = s_1 = 1$.}{
            Let $E$ be the first block in which either world advances. If neither world advances this megablock, let $E = B$. In order for $s_0 = s_1 = 1$ at the end of the megablock, it has to be the case that Bob does not $2$-decode any of Alice's messages after block $E$, meaning that at least $\frac34 - \frac32\epsilon$ of each of Alice's messages after block $E$ are erased.
            
            Prior to block $E$, neither world advanced. For either world, this means that there were at most $i \le n$ blocks in which Alice heard $1$'s followed by $0$'s. In the other $\ge (E-1) - n$ blocks, Alice heard only $1$'s. In such a block, let $V$ be the first chunk in which Bob $2$-decodes Alice's message such that $\rec_0 \vee \rec_1 = \true$, so that he sends $\bar{1}$'s before chunk $V$ and $\bar{0}$'s in or after chunk $V$. Since Alice only hears $1$'s, she does not receive any of Bob's messages in or after chunk $V$. Furthermore, since chunk $V$ was the first chunk in which Bob $2$-decodes Alice's message such that at least one value of $\rec$ was true, in both worlds it must be the case that in all but one chunk before $V$, the adversary erased either $\frac34 - \frac32\epsilon$ of Alice's message or all of Bob's (and $\frac12 - \epsilon$ of Alice's). To summarize, in each of the $\ge (E-1) - n$ blocks, at least 
            \begin{align*}
                \frac{(V-2) \cdot \min \left\{ (\frac34 - \frac32\epsilon) \cdot 4M, (\frac12 - \epsilon) \cdot 4M + M \right\} + (C-V+1) \cdot \left( (\frac12 - \epsilon) \cdot 4M + M \right)}{C \cdot 5M} \\
                \ge \left( \frac35 - \frac65\epsilon \right) \cdot \frac{C-1}{C} \\
                = \left( \frac35 - \frac65\epsilon \right) \cdot \left( 1 - \epsilon \right) \\
                \ge \frac35 - \frac95\epsilon
            \end{align*}
            of the rounds were erased.
            
            Combining this with the fact that after block E, $\frac34 - \frac32\epsilon$ of each of Alice's messages is erased, we get that 
            \begin{align*}
                &\ge \frac{(E - n - 1) \cdot \left( \frac35 - \frac95\epsilon \right) \cdot C \cdot 5M + (B - E) \cdot \left( \frac34 - \frac32\epsilon \right) \cdot C \cdot 4M}{B \cdot C \cdot 5M} \\
                &= \frac{(\frac35 - \frac65\epsilon) \cdot B - \frac35\epsilon E - ( \frac35 - \frac95\epsilon) \cdot (n+1)}{B} \\
                &\ge \left( \frac35 - \frac95\epsilon \right) \left( 1 - \frac{n+1}{B} \right) \\
                &= \left( \frac35 - \frac95\epsilon \right) \left( 1 - \epsilon \right) \\
                &\ge \frac35 - \frac{12}{5}\epsilon
            \end{align*}
            of the megablock must have been erased.
        }
        \case{One world is in Stage $s_b = 1$ and the other in is Stage $s_b = 2$.}{
            Since Bob last saw that one world was in Stage 1 and the other was in Stage 2, he is in Phase 2 at the beginning of this megablock. He just sends $\bar{0}$'s for the rest of the protocol. If Bob doesn't ever $2$-decode a message this megablock in which either world has advanced to Stage 3, this means that in every chunk except for the last in the entire megablock, either Alice's message is $(\frac34 - \frac32\epsilon)$-erased or all of Bob's message was erased along with $\frac12 - \epsilon$ of Alice's. This gives a total of
            \begin{align*}
                &\ge \min \left\{ \frac{\left( \frac34 - \frac32\epsilon \right) \cdot 4M}{5M}, \frac{\left( \frac12 - \epsilon \right) \cdot 4M + M}{5M} \right\} \cdot \left( \frac{B \cdot C - 1}{B \cdot C} \right) \\
                &\ge \left( \frac35 - \frac65\epsilon \right) \cdot \left( 1 - \epsilon \right) \\
                &\ge \frac35 - \frac95\epsilon.
            \end{align*}
        }
        \case{One world is in Stage $s_b = 3$ and the other is in Stage $s_b \in \{ 1, 2 \}$.}{
            The final case is if one state is already in Stage 3, and the other is not. W.l.o.g. suppose $s_0 \in \{ 1, 2 \}$ and $s_1 = 3$. In this case, we simply have to analyze the number of erasures made by the adversary if Alice corresponded to state $0$, that is, her true input were $x_0$.
            
            Let $E$ be the first block in which Alice advances. If she doesn't advance this megablock, let $E = B$. In order for $s_0$ to not have changed at the of the megablock, it has to be the case that Bob does not $2$-decode any of Alice's messages after block E, meaning that at least $\frac34 - \frac32\epsilon$ of each of Alice's messages after block E are erased.
            
            Prior to block E, Alice does not advance. This means that there were at most $j \le n$ blocks in which Alice heard $1$'s followed by $0$'s. In the other $\ge (E-1) - n$ blocks, Alice heard only $1$'s. In such a block, let $V$ be the first chunk in which Bob $2$-decodes Alice's message such that $\rec_0 = \true$, so that he only sends $\bar{1}$'s before chunk $V$ and $\bar{0}$'s in or after chunk $V$. Since Alice only hears $1$'s this block, she does not receive any of Bob's messages in or after chunk $V$. Furthermore, since chunk $V$ was the first chunk in which Bob $2$-decodes Alice's messages such that $\rec_0 = \true$, it must be the case that in all but one chunk before $V$, the adversary erased either $\frac34 - \frac32\epsilon$ of Alice's message or all of Bob's and $\frac12 - \epsilon$ of Alice's. That is, in each of the $\ge (E - 1) - n$ blocks, at least 
            \begin{align*}
                \frac{(V-2) \cdot \min \left\{ (\frac34 - \frac32\epsilon) \cdot 4M, (\frac12 - \epsilon) \cdot 4M + M \right\} + (C-V+1) \cdot \left( (\frac12 - \epsilon) \cdot 4M + M \right)}{C \cdot 5M} 
                \ge \frac35 - \frac95\epsilon
            \end{align*}
            of the rounds were erased.
            
            Combining this with the fact that after block E, $\frac34 - \frac32\epsilon$ of each of Alice's messages is erased, by the same calculation as in Case 1, we get that $\ge \frac35 - \frac{12}{5}\epsilon$ of the megablock must have been erased.
        }
    \end{caseof}
\end{proof}



% \begin{lemma}
%     If Alice does not advance within a megablock, then at least $\frac35 - \frac{12}{5}\epsilon$ of the rounds were corrupted.
% \end{lemma}

% \begin{proof}
%     Suppose Alice does not advance in a megablock. This can happen in two ways: either Bob never sets $\adv = \true$, or Alice never receives a $0$ after Bob has set $\adv = \true$. Let $t$ be the block after which Bob sets $\adv = \true$, or $t = B$ if Bob never sets $\adv = \true$. Then, in blocks $t+1, \dots, B$, Bob's messages are entirely erased, along with $\frac12 - \epsilon$ of each of Alice's messages. Meanwhile, in blocks $1,\dots,t$, $\adv = \false$ so Bob begins each block by sending $\bar{1}$'s, and sends $\bar{0}$'s only to confirm 2-decoded unconfirmed increment(s). Note that if Alice sees a $0$, she confirms her current value of $\cnt$, and the next time she sees a $0$ in a different block she must've incremented $\cnt$ again. Then, since the largest Alice's counter ever gets within the megablock is upper bounded by $i$, there must be at most $i \le n$ blocks among the first $t$ blocks in which she sees a $0$. In each of the other blocks within the first $t$, Alice never sees a $0$. 
    
%     \begin{claim} \label{claim:block}
%         In each such block among the first $t$ blocks where Alice does not see a $0$, at least $\frac35 - \frac95\epsilon$ of the rounds within that block were corrupted.
%     \end{claim}
    
%     \begin{proof}
%         Suppose that Alice does not see a $0$ within a block. In each chunk, Bob sends $\bar{1}$'s until Alice has confirmed reception of a $1$ by setting $\rec = \true$, and then he sends $\bar{0}$'s for the rest of the block. Let $r+1$ be the chunk in which Bob begins sending $\bar{0}$'s, or $r = C$ if Bob never begins sending $\bar{0}$'s. Then, in chunks $r+1,\dots,C$, the adversary must've erased all of Bob's message, along with the necessary $\frac12 - \epsilon$ of Alice's (otherwise Bob can unique-decode Alice's message). Since Bob did not note that $\rec = \true$ sooner, in each of chunks $1,\dots,r-1$, either Alice's message was $(\frac34-\frac32\epsilon)$-erased, or Bob's entire message of $\bar{1}$'s was erased (along with $\frac12-\epsilon$ of Alice's), or both. This means that in every chunk $\in [C] \backslash \{ r \}$, at least
%         \[
%             \min \left\{ \frac{\left( \frac12 - \epsilon \right) \cdot 4M + M}{5M}, \frac{\left( \frac34 - \frac32 \epsilon \right) \cdot 4M}{5M} \right\}
%             = \frac35 - \frac65\epsilon
%         \]
%         of the rounds were corrupted. So, in total, at least
%         \[
%             \frac{\left( \frac35 - \frac65\epsilon \right) \cdot (C-1)}{C}
%             = \left( \frac35 - \frac65\epsilon \right) \cdot \left( 1 - \epsilon \right)
%             \ge \frac35 - \frac95\epsilon
%         \]
%         of the rounds within the block must've been erased.
%     \end{proof}
    
%     This means that the fraction of erasures within a megablock so that Alice does not advance is at least:
%     \begin{align*}
%         \ge \frac{
%             (B-t) \cdot \left( \left( \frac12 - \epsilon \right) \cdot 4M + M \right)
%             + (t-n) \cdot \left( \frac35 - \frac95\epsilon \right) \cdot 5M
%         }{B \cdot 5M} 
%         &= \frac{
%             (\frac35 - \frac45\epsilon) B
%             - \epsilon t 
%             - (\frac35 - \frac95\epsilon) n
%         }{B} \\
%         &\ge \frac{B-n}{B} \cdot \left( \frac35 - \frac95\epsilon \right) \\
%         &= \left( 1 - \epsilon \right) \cdot \left( \frac35 - \frac95\epsilon \right) \\
%         &\ge \frac35 - \frac{12}{5}\epsilon.
%     \end{align*}
% \end{proof}

==> erasure.tex <==
\section{Binary Erasure Channels: Breaking the $1/2$ Barrier} \label{sec:erasure}

% In this section, we discuss the optimal erasure resilience of interactive one-way protocols. In particular, we display an efficient (polynomial-blowup in communication) construction that achieves an error resilience of $\frac47$ (Section~\ref{sec:4/7}), and an inefficient (exponential-blowup in communication) construction that achieves an error resilience of $\frac35$ (Section~\ref{sec:3/5}). We begin in Section~\ref{sec:6/11} by presenting a simpler scheme that achieves an error resilience of $\frac{6}{11}$; this scheme provides the basic structure of our optimized protocols.

Classical error-correcting codes cannot achieve an erasure resilience $>\frac12$.\mnote{should we cite this...} In this section, we present the main result of our paper: an efficient (polynomial-blowup in communication) interactive error-correcting code that achieves an adversarial error resilience greater than $\frac12$. In particular, our protocol achieves an error resilience of $\frac35$ (Section~\ref{sec:3/5}). We begin in Section~\ref{sec:6/11} by presenting a simpler scheme that achieves an error resilience of $\frac{6}{11}$; this scheme provides the basic structure of our optimized protocol.

\input{erasure/6.11-construction}

% \input{erasure/4.7-construction}

\input{erasure/3.5-construction}

% \input{erasure/2.3-upper-bound}

==> intro-old.tex <==
\section{Introduction}

Consider the following task: Alice wishes to communicate a message to Bob such that even if a constant fraction of the communicated bits are adversarially tampered with, Bob is still guaranteed to be able to determine her message. This task motivated the prolific study of \emph{error correcting codes}, starting with the seminal works of~\cite{Shannon48,Hamming50}. An error correcting code encodes a message $x$ into a longer codeword $\ECC(x)$, such that the Hamming distance between any two distinct codewords is a constant fraction of the length of the codewords. To communicate a message $x$, Alice sends Bob the corresponding codeword $\ECC(x)$, and the fact that the distance between any two codewords is large guarantees that an adversary must corrupt a large fraction of the communication in order for Bob to decode to the wrong codeword. 

An important question in the study of error correcting codes is determining the maximal possible error resilience.  Indeed, many works focus on precisely this question.  In general, the error resilience parameter depends on the alphabet size: in this work we focus on the binary alphabet.  Two main error models are considered in the literature:  The bit-flip model, where the adversary can flip a constant fraction of the bits of the codeword, and the erasure model, where the adversary can erase a constant fraction of the bits of the codeword (where each erased bit is replaced by a special erasure symbol).\footnote{Another common model that was considered is the insertion/deletion model, which we do not address in this work.}  It is known that in the adversarial bit-flip model, any $\ECC$ can be resilient to at most $\frac14$ corruptions, and in the adversarial erasure error model any $\ECC$ can be resilient to at most $\frac12$ corruptions.

In this work, we investigate the following natural question:

\begin{center}
{\em Can we achieve better error resilience if we use interaction?}\footnote{We note that a related question was previously asked in the setting of $\ECC$ with feedback~\cite{Berlekamp68,Zigangirov76,SpencerW92,AhlswedeDL06,BravermanE14,HaeuplerKV15,WangQC17}; we elaborate on these works in Section~\ref{sec:related:feedback}. }
\end{center}

We show that interaction can be used to boost the error rate beyond the realm of what is possible using (non-interactive) error correcting codes.  Specifically, we show that there is a way for Alice to communicate $x$ to Bob such that Bob is guaranteed to learn $x$ \emph{even if $\approx \frac35$ of the total communicated bits are erased!} 

This result essentially shows that Bob talking occasionally \emph{instead of Alice} actually improves the error resilience. It is not obvious that this should be the case!  In particular, Bob can only send ``feedback'' since he has no input of his own, while Alice can actually send new information. Thus Bob's messages seem less valuable than Alice's. How can the error resilience be improved when messages containing information about $x$ have been replaced by messages without? We emphasize that Bob's feedback messages may be corrupted as well, thus making Alice obtain the incorrect feedback.\footnote{Jumping ahead, we note that the main difference between our work and the works on $\ECC$ with feedback (discussed in Section~\ref{sec:related:feedback}) is that we allow the feedback to be {\em arbitrarily} corrupted, and the cost of corrupting the messages from Alice is the same as corrupting the feedback from Bob.} Nevertheless, we show that these feedback messages play a vital role in increasing the error resilience past $\frac12$. 



% We note that interaction has been considered in the context of error resilience starting with the seminal works of Shculman~\cite{?,?,?}.  However, in these works, and all followup works, interaction was viewed as a difficult reality that we need to deal with, as oppposed to a tool.  In other word, these works considered the task of taking an interactive protocol and making it error resilient.
% In this work, we revert to the standard message transmission task, where a party wishes to send a single message to another other party.  Our goal is to improve the error resilience beyond what is possible with (standard) $\ECC$s.

\paragraph{Interactive error correcting codes.}  We call an interactive protocol where Alice communicates $x$ to Bob an \emph{interactive error correcting code ($\iECC$)}, defined formally in Section~\ref{iecc-def}.\footnote{We empasize that this notion differs from the notion of interactive coding (elaborated on in Section~\ref{sec:IC}), in that an $\iECC$ sends a {\em single} message  via an interactive protocol, whereas interactive coding converts an {\em interactive protocol} into an error reslient one.}  An $\iECC$ is an interactive protocol with a fixed length (number of rounds) and fixed speaking order, where in a given round the designated party sends exactly one bit, and Bob is guaranteed to correctly learn Alice's input $x$ at the end, provided not too many bits were corrupted. Note that a classical error correcting code is an $\iECC$ in which Alice speaks in every round. 

%We argue that considering this interactive variant of an error correcting code is very natural. Indeeed, interaction has been considered in other (originally non-interactive) tasks, such as proof systems, starting in the mid eighties \cite{GMR85}. % We thus find it quite surprizing that interactive $\ECC$ were not previously studied, except in the setting where the underlying error-free communication is interactive \cite{Schulman92,Schulman93,Schulman96} (we elaborate on this line of work in Section~\ref{sec:IC}). 


We view $\iECC$'s as a natural solution to the original task of Alice communicating a message $x$ to Bob under adversarial erasure. 
% We are surprised that our notion of an $\iECC$ has not been presented before. It is the most natural way to address the original task of Alice communicating a message $x$ to Bob, under the most natural definition of adversarial error. 
As mentioned above, we construct $\iECC$'s that provide better error resilience (under adversarial erasure) than traditional $\ECC$'s, thus demonstrating that they \emph{are more powerful} than traditional $\ECC$'s. But there may be many other potential benefits they may have over traditional $\ECC$'s. Can $\iECC$'s achieve better error rate in other error models (such as the bit-flip model or the random error model)?  Can they achieve a better  communication rate? Do $\iECC$'s have any practical advantages?  We leave these questions to investigation in future work. 

%Perhaps surprisingly, by leveraging the power of interaction, we design an $\iECC$ that is resilient to $\approx\frac35$ adversarial erasures. As such, our result shows that interactive error correcting codes are in fact more powerful than classical error correcting codes.





%By the Gilbert-Varshamov bound, the best possible relative distance\footnote{\ynote{Why are we getting into this?} The relative distance of an error-correcting code is the maximum possible minimum distance between two codewords, as the number of codewords approaches $\infty$. In general, when we talk about relative distance or error resilience, we mean as the number of possible messages $x$ approaches $\infty$.} of any error correcting code over the binary alphabet is $\le \frac12$. Since the relative distance of an error correcting code is precisely its resilience to adversarial erasures, this means that to communicate $x$ to Bob over a binary channel, if Alice simply sends an error correcting code, she can be resilient to at most $\frac12$ adversarial erasures, but no more. Whether there exists a protocol with resilience to $> \frac12$ adversarial erasures was previously unknown.
% Over large alphabets, there are known constructions of error correcting codes that achieve distance $\approx 1$. \mnote{i'm not actually sure it makes sense to mention large alphabet at all. weak opinion though. } Over the binary alphabet, however, the best possible distance of any error correcting code is $\le \frac12$, by the Gilbert-Varshamov bound.\mnote{we do need to get across here or somewhere else that we mean limit is 1/2 as Alice's input size gets large.} In the case of erasures, the distance of an error correcting code is precisely its resilience to adversarial erasures. 
% This means that to commuicate $x$ to Bob over a binary channel, if Alice simply sends an error correcting code, she can be resilient to at most $\frac12$ adversarial erasures, but no more.
% \mnote{Feel free to reword, but the general sentiment is that ``simply sending an ECC'' doesn't sound right.}
% Whether there exists a protocol with resilience to $> \frac12$ adversarial erasures was previously unknown.



\subsection{Our Results.}

Our main result is an $\iECC$ that achieves an erasure resilience of $\frac35$ over the binary erasure channel.
\begin{theorem}
    For any $\epsilon > 0$, there exists an $\iECC$ over the binary erasure channel resilient to $\frac35-\epsilon$ erasures, such that the communication complexity for inputs of size $n$ is $O_\epsilon(n^2)$.
\end{theorem}


We also prove the following impossibility result.

\begin{theorem} \label{thm:intro-2/3}
    There does not exist an $\iECC$ over the binary erasure channel resilient to $\frac23$ erasures.
\end{theorem}

We also consider the problem of constructing an $\iECC$ over the binary \emph{bit flip} channel. In this setting, instead of erasing bits, an adversary may toggle bits of her choice. 
We do not know of any constructions of $\iECC$s that achieve a higher error resilience to bit flips than the standard (non-interactive) error correcting code (which achieves a maximal error rate of $\frac14$). We leave open the problem of constructing such an $\iECC$.
%By using a classical error correcting code with distance $\frac12$, we can construct a trivial $\iECC$ resilient to $\frac14$ adversarial bit flips.
We prove the following negative result on the maximal possible error resilience to bit flips of any $\iECC$ scheme.

\begin{theorem} \label{thm:intro-2/7}
    There does not exist an $\iECC$ over the binary bit flip channel resilient to $\frac27$ adversarial bit flips.
\end{theorem}



\input{intro/related}

\input{intro/technical-overview}

==> intro-old2.tex <==
\section{Introduction}

Consider the following task: Alice wishes to communicate a message to Bob such that even if a constant fraction of the communicated bits are adversarially tampered with, Bob is still guaranteed to be able to determine her message. This task motivated the prolific study of \emph{error correcting codes}, starting with the seminal works of~\cite{Shannon48,Hamming50}. An error correcting code encodes a message $x$ into a longer codeword $\ECC(x)$, such that the Hamming distance between any two distinct codewords is a constant fraction of the length of the codewords. To communicate a message $x$, Alice sends Bob the corresponding codeword $\ECC(x)$, and the fact that the distance between any two codewords is large guarantees that an adversary must corrupt a large fraction of the communication in order for Bob to decode to the wrong codeword. 

An important question in the study of error correcting codes is determining the maximal possible error resilience.  Indeed, many works focus on precisely this question.  In general, the error resilience parameter depends on the alphabet size: in this work we focus on the binary alphabet.  Two main error models are considered in the literature:  The bit-flip model, where the adversary can flip a constant fraction of the bits of the codeword, and the erasure model, where the adversary can erase a constant fraction of the bits of the codeword (where each erased bit is replaced by a special erasure symbol).\footnote{Another common model that was considered is the insertion/deletion model, which we do not address in this work.}  It is known that in the adversarial bit-flip model, any $\ECC$ can be resilient to at most $\frac14$ corruptions, and in the adversarial erasure error model any $\ECC$ can be resilient to at most $\frac12$ corruptions.

In this work, we investigate the following natural question:

\begin{center}
{\em Can we achieve better error resilience if we use interaction?}
\end{center}

This question is what motivated the study of {\em $\ECC$'s with feedback} \cite{Berlekamp64,Berlekamp68,Zigangirov76,SpencerW92,AhlswedeDL06,HaeuplerKV15}, where after every bit sent the sender receives some information about the bits the receiver has received so far. This feedback cannot be corrupted and is not counted towards the adversary's budget. That is, the error resilience is measured as a fraction of Alice's forward communication.

In many applications, however, feedback may be corrupted just as forward communication is corrupted. We propose the new model of {\em interactive error correcting codes} ($\iECC$), which does not distinguish between the forward rounds and the feedback rounds; rather the adversary is given an budget which is an $\alpha$-fraction of the {\em total} communication (for some $\alpha>0$), which she can spend {\em arbitrarily} (e.g., all on forward communication, or on some combination of forward and feedback communication).

% This question is what motivated the study of {\em $\ECC$'s with noiseless feedback} \cite{Berlekamp64,Berlekamp68,Zigangirov76,SpencerW92,AhlswedeDL06,HaeuplerKV15}, where after every bit sent the sender receives some information about the bits the receiver has received so far. This feedback cannot be corrupted and is not counted towards the adversary's budget. 
% However, in all works considering feedback, feedback rounds are treated differently than forward rounds in terms of calculating error resilience. In particular, there is a separate corruption budget for forward and feedback rounds (most often, the feedback rounds are used as free additional power to Alice: they cannot be corrupted and are not counted to the corruption budget at all). \mnote{want to figure out more about what ECC's with feedback have been considered before}

% In many applications, however, feedback may be corrupted just as forward communication is corrupted. Little is known about the power of noisy feedback with adversarial corruptions. Existing works either replace the adversary with the binary symmetric channel~\cite{BurnashevY08a,BurnashevY08b} or construct schemes over large alphabets~\cite{WangQC17}; in the latter case they impose a separate corruption budget for forward and feedback rounds. 

% In our work, we make progress on analyzing the power of noisy feedback in the case of adversarial binary erasures. 

% Treating corruptions on forward and feedback rounds separately does not capture the full generality of the adversary, but is critical in all existing works on $\ECC$'s with noiseless or noisy feedback.
% In our paper, we make the first breakthrough with a fully general adversary. We define the model of {\em interactive error correcting codes} ($\iECC$), which does not distinguish between the forward rounds and the feedback rounds; rather the adversary is given an budget which is an $\alpha$-fraction of the {\em total} communication (for some $\alpha>0$), which she can spend {\em arbitrarily} (e.g., all on forward communication, or on some combination of forward and feedback communication).

This question is what motivated the study of {\em $\ECC$'s with feedback} \cite{Berlekamp64}, where after every bit sent the sender receives some information about the bits the receiver has received so far. This feedback can either be noiseless~\cite{Berlekamp68,Zigangirov76,SpencerW92,AhlswedeDL06,HaeuplerKV15} or noisy~\cite{WangQC17}. However, in all works considering feedback, feedback rounds are treated differently than forward rounds in terms of calculating error resilience. In particular, there is a separate corruption budget for forward and feedback rounds (most often, the feedback rounds are used as free additional power to Alice: they cannot be corrupted and are not counted to the corruption budget at all). 

This imposition of a separate corruption budget for the forward and feedback rounds does not capture the full generality of the adversary, but is critical in all existing constructions improving erasure resilience beyond $\frac12$ or bit flip resilience beyond $\frac14$. In our paper, we make the first breakthrough with a fully general adversary. We define the model of {\em interactive error correcting codes} ($\iECC$), which does not distinguish between the forward rounds and the feedback rounds; rather the adversary is given an budget which is an $\alpha$-fraction of the {\em total} communication (for some $\alpha>0$), which she can spend {\em arbitrarily} (e.g., all on forward communication, or on some combination of forward and feedback communication).

Quite surprisingly, we show that even this model allows us to boost the erasure resilience of the protocol beyond $\frac12$. In particular, we show that there is an $\iECC$ for which Bob correctly learns Alice's message $x$ \emph{even if $\frac35$ of the total communication is erased!} 

We view $\iECC$'s as the most general and natural solution to the original task of Alice communicating a message $x$ to Bob under adversarial erasure.\footnote{Recall that the $\ECC$ with feedback model makes the additional assumption that Alice's forward messages and Bob's feedback messages are corrupted separately which is critical in constructions which improve error resilience.} Note that a standard (non-interactive) $\ECC$ is an $\iECC$ in which Alice speaks in every round. Our result essentially shows that Bob talking occasionally \emph{instead of Alice} actually improves the erasure resilience. It is not obvious that this should be the case! In particular, Bob can only send feedback since he has no input of his own, while Alice can actually send new information. Thus Bob's messages seem less valuable than Alice's. How can the erasure resilience be improved when messages containing information about $x$ have been replaced by messages without? Nevertheless, we show that these feedback messages play a vital role in increasing the erasure resilience past $\frac12$. 

% Compare this to $\ECC$'s with feedback, in which Bob talks \emph{in addition to} Alice. Since the forward and feedback rounds are treated separately, feedback can never hurt. As a result, it is not surprising that $\ECC$'s with feedback would be able to improve erasure resilience. 
% On the other hand, in our model of $\iECC$'s, Bob talks \emph{instead of} Alice, as his feedback rounds contribute to the same collective corruption budget as Alice's messages.
% Bob talks \emph{instead of} Alice, as his feedback rounds contribute to the same corruption budget as Alice's messages. 
% In particular, the adversary can use budget gained via Bob's less useful feedback rounds to corrupt Alice's more useful forwards rounds. Preventing this is precisely why the works on $\ECC$ with feedback used such a critical assumption. Nevertheless, we show that these feedback messages play a vital role in increasing the erasure resilience past $\frac12$. 
% Our result essentially shows that Bob talking occasionally \emph{instead of Alice} actually improves the erasure resilience. 
% It is not obvious that replacing Alice's forward messages with Bob's feedback rounds should be powerful enough to improve the erasure resilience! In particular, Bob can only send feedback since he has no input of his own, while Alice can actually send new information. Thus Bob's messages seem less valuable than Alice's. How can the erasure resilience be improved when messages containing information about $x$ have been replaced by messages without? 
% Nevertheless, we show that these feedback messages play a vital role in increasing the erasure resilience past $\frac12$. 

% In other words, we remove the assumption from the $\ECC$ with feedback models that requires that the adversary split their corruption between the forward and feedback rounds. Even with a fully general adversary who can use budget gained via the feedback rounds to corrupt the forward rounds, which likely contain more valuable information, we can improve the erasure resilience beyond $\frac12$!

% \paragraph{Interactive Error Correcting Codes.} More precisely, an $\iECC$ consists of a fixed length (number of rounds) and fixed speaking order, where in a given round the designated party sends exactly one bit, and Bob is guaranteed to correctly learn Alice's input $x$ at the end, provided that the {\em total} number of bits corrupted is not too large.\footnote{Note that a classical error correcting code is an $\iECC$ in which Alice speaks in every round.} We construct an $\iECC$ in which Bob is guaranteed to learn Alice's message $x$ \emph{even if $\frac35$ of the communicated bits are erased!}

As mentioned above, we demonstrate that  $\iECC$'s \emph{are more powerful} than traditional $\ECC$'s by constructing an $\iECC$ that provides better error resilience for adversarial erasure corruptions. But there may be many other potential benefits they may have over traditional $\ECC$'s. Can $\iECC$'s achieve better error rate in other error models (such as the bit-flip model)? 
% Can they achieve a better communication rate? 
Do $\iECC$'s have any practical advantages?  We leave these questions to investigation in future work. 


%\ynote{slightly reworded from here until Section 1.1, tried to address Meghal's comment}
%A related line of work is that \mnote{this question is what motivated the study } of {\em $\ECC$ with feedback} \cite{Berlekamp64}, where after every bit sent the sender receives some information about the bits the receiver has received so far. This feedback can either be noiseless~\cite{Berlekamp68,Zigangirov76,SpencerW92,AhlswedeDL06,HaeuplerKV15} or noisy~\cite{BravermanE14,WangQC17}. However, in all works considering feedback, feedback rounds are treated differently than forward rounds in terms of calculating error resilience. In particular, either the feedback rounds are counted as free, i.e. the corruption budget is measured as a fraction of only the forward rounds, or there is a separate corruption budget for forward and feedback rounds.


 %In our work, we consider a different model, in which both forward and feedback rounds are counted \emph{equally} \mnote{the word equally doesn't express the right sentiment.} towards the corruption budget. \mnote{ the paragraph as written is not very powerful. It just says here's a model for feedback that is different than existing ones, without motivating why it is interesting.}





%\paragraph{Interactive error correcting codes.}  
%We define the model of {\em interactive error correcting codes} ($\iECC$), which does not  discriminate between the forward rounds and the feedback rounds; rather the adversary is given an budget which is an $\alpha$-fraction of the {\em total} communication (for some $\alpha>0$), which she can spend {\em arbitrarily} (e.g., all on forward communication, or on some combination of forward and feedback communication).

%Quite surprisingly, we show that even this model allows to boost the error rate beyond the realm of what is possible using (non-interactive) error correcting codes. It is not all that surprising that the $\ECC$ with feedback model allows for this -- since the forward and feedback rounds are treated separately, feedback can never hurt. However, in our model, the adversary can use budget gained via the feedback rounds to corrupt the forward rounds, which likely contain less valuable information! This is precisely why the works on $\ECC$ with feedback treated the feedback messages differently from Alice's messages! We show that even in the $\iECC$ model (which does not discriminate between forward and feedback messages) these feedback messages play a vital role in increasing the error resilience past $\frac12$. 
%This result essentially shows that Bob talking occasionally \emph{instead of Alice} actually improves the error resilience. It is not obvious that this should be the case!  
%The reason this may seem surprising at first is that the feedback rounds seem less valuable than the forward rounds, which actually contain new information. Namely, how can the error resilience be improved when messages containing information about $x$ have been replaced by messages without? This is precisely why the works on $\ECC$ with feedback treated the feedback messages differently from Alice's messages! We show that even in the $\iECC$ model (which does not discriminate between forward and feedback messages) these feedback messages play a vital role in increasing the error resilience past $\frac12$. 

%More precisely, an $\iECC$ consists of a fixed length (number of rounds) and fixed speaking order, where in a given round the designated party sends exactly one bit, and Bob is guaranteed to correctly learn Alice's input $x$ at the end, provided that the {\em total} number of bits corrupted is not too large.\footnote{Note that a classical error correcting code is an $\iECC$ in which Alice speaks in every round.}   
%We show that this interaction can be used to boost the error rate, %beyond the realm of what is possible using (non-interactive) error correcting codes. 
%We construct an $\iECC$ in which Bob is guaranteed to learn Alice's message $x$ \emph{even if $\frac35$ of the communicated bits are erased!}





% We note that interaction has been considered in the context of error resilience starting with the seminal works of Shculman~\cite{?,?,?}.  However, in these works, and all followup works, interaction was viewed as a difficult reality that we need to deal with, as oppposed to a tool.  In other word, these works considered the task of taking an interactive protocol and making it error resilient.
% In this work, we revert to the standard message transmission task, where a party wishes to send a single message to another other party.  Our goal is to improve the error resilience beyond what is possible with (standard) $\ECC$s.

% \paragraph{Interactive error correcting codes.}  We call an interactive protocol where Alice communicates $x$ to Bob an \emph{interactive error correcting code ($\iECC$)}, defined formally in Section~\ref{iecc-def}.\footnote{We empasize that this notion differs from the notion of interactive coding (elaborated on in Section~\ref{sec:IC}), in that an $\iECC$ sends a {\em single} message  via an interactive protocol, whereas interactive coding converts an {\em interactive protocol} into an error reslient one.}  An $\iECC$ is an interactive protocol with a fixed length (number of rounds) and fixed speaking order, where in a given round the designated party sends exactly one bit, and Bob is guaranteed to correctly learn Alice's input $x$ at the end, provided not too many bits were corrupted. Note that a classical error correcting code is an $\iECC$ in which Alice speaks in every round. 

%We argue that considering this interactive variant of an error correcting code is very natural. Indeeed, interaction has been considered in other (originally non-interactive) tasks, such as proof systems, starting in the mid eighties \cite{GMR85}. % We thus find it quite surprising that interactive $\ECC$ were not previously studied, except in the setting where the underlying error-free communication is interactive \cite{Schulman92,Schulman93,Schulman96} (we elaborate on this line of work in Section~\ref{sec:IC}). 


%We view $\iECC$'s as a natural solution to the original task of Alice communicating a message $x$ to Bob under adversarial erasure. 
% We are surprised that our notion of an $\iECC$ has not been presented before. It is the most natural way to address the original task of Alice communicating a message $x$ to Bob, under the most natural definition of adversarial error. 
%As mentioned above, we demonstrate that  $\iECC$'s  \emph{are more powerful} than traditional $\ECC$'s by constructing an $\iECC$ that provide better error resilience for adversarial erasure corruptions.    
%But there may be many other potential benefits they may have over traditional $\ECC$'s. Can $\iECC$'s achieve better error rate in other error models (such as the bit-flip model or the random error model)?  Can they achieve a better  communication rate? Do $\iECC$'s have any practical advantages?  We leave these questions to investigation in future work. 

%Perhaps surprisingly, by leveraging the power of interaction, we design an $\iECC$ that is resilient to $\approx\frac35$ adversarial erasures. As such, our result shows that interactive error correcting codes are in fact more powerful than classical error correcting codes.





%By the Gilbert-Varshamov bound, the best possible relative distance\footnote{\ynote{Why are we getting into this?} The relative distance of an error-correcting code is the maximum possible minimum distance between two codewords, as the number of codewords approaches $\infty$. In general, when we talk about relative distance or error resilience, we mean as the number of possible messages $x$ approaches $\infty$.} of any error correcting code over the binary alphabet is $\le \frac12$. Since the relative distance of an error correcting code is precisely its resilience to adversarial erasures, this means that to communicate $x$ to Bob over a binary channel, if Alice simply sends an error correcting code, she can be resilient to at most $\frac12$ adversarial erasures, but no more. Whether there exists a protocol with resilience to $> \frac12$ adversarial erasures was previously unknown.
% Over large alphabets, there are known constructions of error correcting codes that achieve distance $\approx 1$. \mnote{i'm not actually sure it makes sense to mention large alphabet at all. weak opinion though. } Over the binary alphabet, however, the best possible distance of any error correcting code is $\le \frac12$, by the Gilbert-Varshamov bound.\mnote{we do need to get across here or somewhere else that we mean limit is 1/2 as Alice's input size gets large.} In the case of erasures, the distance of an error correcting code is precisely its resilience to adversarial erasures. 
% This means that to commuicate $x$ to Bob over a binary channel, if Alice simply sends an error correcting code, she can be resilient to at most $\frac12$ adversarial erasures, but no more.
% \mnote{Feel free to reword, but the general sentiment is that ``simply sending an ECC'' doesn't sound right.}
% Whether there exists a protocol with resilience to $> \frac12$ adversarial erasures was previously unknown.



\subsection{Our Results.}

Our main result is an $\iECC$ that achieves an erasure resilience of $\frac35$ over the binary erasure channel.
\begin{theorem}
    For any $\epsilon > 0$, there exists an $\iECC$ over the binary erasure channel resilient to $\frac35-\epsilon$ erasures, such that the communication complexity for inputs of size $n$ is $O_\epsilon(n^2)$.
\end{theorem}


We also prove the following impossibility result.

\begin{theorem} \label{thm:intro-2/3}
    There does not exist an $\iECC$ over the binary erasure channel resilient to $\frac23$ erasures.
\end{theorem}

We also consider the problem of constructing an $\iECC$ over the binary \emph{bit flip} channel. In this setting, instead of erasing bits, an adversary may toggle bits of her choice. 
We do not know of any constructions of $\iECC$s that achieve a higher error resilience to bit flips than the standard (non-interactive) error correcting code (which achieves a maximal error rate of $\frac14$). We leave open the problem of constructing such an $\iECC$.
%By using a classical error correcting code with distance $\frac12$, we can construct a trivial $\iECC$ resilient to $\frac14$ adversarial bit flips.
We prove the following negative result on the maximal possible error resilience to bit flips of any $\iECC$ scheme.

\begin{theorem} \label{thm:intro-2/7}
    There does not exist an $\iECC$ over the binary bit flip channel resilient to $\frac27$ adversarial bit flips.
\end{theorem}



\input{intro/related}

\input{intro/technical-overview}

==> intro/overview-short.tex <==
\subsection{Technical Overview} \label{sec:overview}

In this overview, we focus our efforts on our construction of an $\iECC$ with an erasure resilience of $> \frac12$. For the lower bounds given in Theorems~\ref{thm:intro-2/3} and~\ref{thm:intro-2/7}, we refer the reader to Sections~\ref{sec:2/3} and~\ref{sec:2/7} respectively for the proofs. 

\subsubsection{A Simpler $6/11$ $\iECC$}

We begin by discussing a simpler scheme that achieves an error resilience over the binary erasure channel of $\frac6{11}$. The overarching goal of our protocol is to perform the following three steps.

\begin{enumerate}
    \item Bob learns that Alice's value of $x$ is one of two possible values. (This idea is known as list decoding, which achieves better noise resilience than unique decoding.) 
    \item Bob conveys to Alice an index $i$ on which the two possible inputs differ.
    \item Alice sends the value of her input on index $i$.
\end{enumerate}

A naive approach to this might be as follows: Alice sends $\ECC(x)$, Bob list-decodes it even with $>\frac12$ erasures, Bob conveys an index to Alice magically, then ...

Our protocol consists of many \emph{chunks} where Alice sends Bob a fixed length message, then Bob sends Alice a fixed length message. The protocol will make \emph{progress} towards the three steps every time a chunk has $<\frac6{11}$ erasures. As long as there are many chunks total, there are also be many chunks with $<\frac6{11}$ erasures. As such, there will eventually be enough progress to complete all three steps.

Before diving into the description, we set up some of the framework. In each chunk Alice sends a message of length $M$ and Bob replies with a message of length $\frac38M$. Alice's possible message space will be $\ECC(x,\cnt) \cup \{0^M,1^M\}$ where $x$ is her input and $\cnt$ is her current guess for $i$, which are all $\frac12$ apart. Bob's messages are all in $\{\}$ which are all distance $\frac23$ apart. Using this message space allows the following three facts to hold true.
\begin{itemize}
    \item If there are $<\frac12$ erasures to Alice's message, Bob can uniquely decode it.
    \item If there are $<\frac34$ erasures to Alice's message, Bob can list-decode it to two options.
    \item If there are $<\frac23$ erasures to Alice's message, Alice can uniquely decode it.
\end{itemize}
Since we are in the setting of erasures, this message (resp. set of messages) is guaranteed to be (resp. contain) the correct message! There is an unambiguous guarantee of this, which is one major advantage of the erasure setting. 

Returning to the $\frac6{11}$ error resilience, this choice implies the following given the $8:3$ message ratio of Alice and Bob: in a chunk with $<\frac6{11}$ erasures, it is guaranteed that either Bob hears $>\frac12$ of Alice's message, or he hears $>\frac14$ of Alice's message \emph{and} Alice hears $>\frac13$ of Bob's message. As such, we have set up a structure with the following important property: \emph{there are many chunks where either Bob uniquely decodes Alice's message, or Bob list-decodes Alice's message to two options, and Alice uniquely decodes Bob's message.}


In our protocol, it is the case that if Bob is ever able to uniquely decode Alice's message, then since we are in the erasure model he knows that the message must be what Alice sent, so he can correctly learn $x$. Otherwise, there are many chunks in the protocol in which Bob can narrow down Alice's message to two options and Alice can uniquely decode Bob's. At each such chunk, progress is made towards Bob learning $x$.


\paragraph{Our protocol.} We finally describe the actual protocol Alice and Bob use to make progress in each such chunk. Note that they can only send message in their respective message spaces, which is especially restrictive for Bob, who can only send a constant number of words. 

In addition to her input $x$, Alice keeps track of a counter $\cnt$ initially set to $0$ indicating her guess for $i$. At the beginning of the protocol, Alice sends $\ECC(x, \cnt)$ to Bob in every chunk. At some point there will be $<\frac6{11}$ erasures in a chunk, and so Bob list decodes Alice's message to at most two options, say $(x_0, \cnt_0 = 0)$ and $(x_1, \cnt_1 = 0)$. Then, Alice's true input must be $x_0$ or $x_1$. Note that if instead Bob uniquely decodes Alice's message, he can unambiguously determine her input $x$ (even if one of those options is $0^M$ or $1^M$ as will become clear later). In general, the case where Bob uniquely decodes Alice's message even later in the protocol allows him to trivially determine $x$, so we do not mention it, and assume that in all chunks with $<\frac6{11}$ error, Bob list-decodes Alice's message to two options, and Alice uniquely decodes Bob's message.

At this point, Bob tries to communicate $i$ to Alice. He cannot simply send $i$, because he is only allowed 4 possible messages. Instead, Bob communicates $i$ to Alice via an \emph{incrementation procedure} where Bob always sends one of his allotted codewords $\bar{0}, \bar{1}$. Alice keeps track of a counter $\cnt$ initially set to $0$, which as we said before indicates her guess for $i$.

As a first attempt, one could consider a scheme in which Alice increments $\cnt$ every time she hears $\bar{1}$ from Bob, and stops incrementing when she hears a $\bar{0}$ from Bob. However, what is Bob to do if he doesn't hear Alice? He doesn't know if she has incremented enough yet so he should send $\bar{0}$, or if she should increment again so he should send $\bar{1}$. If he sends $\bar{1}$ every time he isn't sure, Alice could increment past $i$. If he sends $\bar{0}$, the adversary could choose not to corrupt this new message, no progress is made when Alice hears the $\bar{0}$.

Instead we use a completely different incrementation procedure: Alice increments only when she detects a \emph{change} in Bob's message from $\bar{0}$ to $\bar{1}$ or vice versa. Meanwhile, Bob sends the same message $\bar{0}$ or $\bar{1}$ until he detects that Alice has incremented, before switching to sending the other codeword. This way, Alice and Bob stay on the same page with the value of $\cnt$, and Alice can never skip over $i$.

Now in every chunk where Bob hears Alice's $\cnt$ and Alice uniquely decodes Bob's message, they can make progress towards incrementing $\cnt$. This is almost like our gurantee for $<\frac6{11}$ error, except Bob actually sees $(x_0,\cnt_0)$ and $(x_1,\cnt_1)$ and the counters $\cnt_0$ and $\cnt_1$ may not be equal! If they are different, Bob will learn the correct $x$ in a different way, addressed later. When they are the same, the procedure will progress, eventually $i$ times, and Alice will reach the index $i$.

When Bob sees that Alice's counter has reached the index $i$, he begins sending a third codeword $\bar{2}$ to ask Alice for the value of her input at index $i$. Upon uniquely decoding $\bar{2}$ (which will happen, since eventually there is a chunk where Bob hears two options and she hears one), Alice knows that the index $i$ has been reached and begins sending $x[i]$ for the rest of the protocol. Once Bob has begun sending $\bar{2}$'s forever, note that Alice will never increment $\cnt$ again, since she only increments when she unambiguously receives a $\bar{0}$ or $\bar{1}$ from Bob. Thus, as long as Alice unambiguously receives $\bar{2}$ at some point, she will have correctly learned $i$ and begins sending the requested value of $x[i]$.
Indeed, if Bob never list decodes to $(x_0, \cnt_0)$ and $(x_1, \cnt_1)$ with $\cnt_0 \not= \cnt_1$, then the above techniques work and are sufficient for Alice to learn the index $i$ correctly.

Recall, however, that at some point Bob may have decoded counters $\cnt_0\neq\cnt_1$. If the counters ever get out of sync, they must be off by $1$, since if the first time the counters get out of sync one is at least $2$ greater than the other, then Bob can conclude that one made an impossible increment and thus deduce $x$. In this case, Bob can begin sending a fourth codeword $\bar{3}$, asking Alice to tell him the parity of her counter. 
% Once again, note that this halts the counting process, as Alice will never again unambiguously decode $\bar{0}$ or $\bar{1}$.

At the end of the protocol, as long as Bob receives at least one bit of Alice's answer to his question (value of $x[i]$, corresponding to $\bar{2}$, or parity of $\cnt$, corresponding to $\bar{3}$), he can correctly deduce Alice's input $x$.  We refer the reader to \cref{sec:6/11} for more details, and a formal description of the protocol and its analysis.
        
For a more formal statement and analysis of this $6/11$ protocol, we refer the reader to Section~\ref{sec:6/11}. This section also includes an informal outline of Alice and Bob's procedures.


\subsubsection{Improving $6/11$ to $3/5$}

In the above protocol, Bob uses two different codewords to increment Alice's counter. Then, when he wants to ask Alice for either the value of $x[\cnt]$ or the parity of $\cnt$, he has to use two \emph{new} codewords to convey the appropriate question. 
If we were able to somehow have Bob use only two codewords, the relative distance between Bob's codewords could increase to $1$. Then, by letting Alice and Bob speak in a $4:1$ ratio, to prevent progress an adversary would have to either corrupt $\frac34$ of Alice's message, or all of Bob's and $\frac12$ of Alice's. This increases the erasure resilience to
\[
    \frac{\frac34 \cdot 4M}{4M + M} = \frac{M + \frac12 \cdot 4M}{4M + M} = \frac35.
\]

In order to get rid of the need for the extra two codewords $\bar{2}$ and $\bar{3}$, we need for the two codewords $\bar{0}$ and $\bar{1}$ to be able to take on \emph{more than two meanings}. To do this, we combine our two codewords with \emph{timing cues}, such that $\bar{0}$ and $\bar{1}$ mean different things depending on where they are heard in the protocol. More specifically, we divide the protocol into \emph{blocks} of chunks,
% To encapsulate the meanings of $\bar{2}$ and $\bar{3}$ with just two codewords $\bar{0} = 0^M$ and $\bar{1} = 1^M$, the main idea is to have $\bar{0}$ and $\bar{1}$ mean different things at different points in the protocol. Let us divide the protocol into \emph{blocks} of chunks, 
% such that it means something different whether Alice hears only $\bar{1}$'s within a block, $\bar{1}$'s followed by $\bar{0}$'s within a block, or $\bar{0}$'s only within a block.
% to the meaning of $\bar{0}$ and $\bar{1}$ depend on whether Alice first hears a $\bar{0}$ or $\bar{1}$ within each block. %The first $\bar{0}$ or $\bar{1}$ in a block will help convey $\bar{2}$ or $\bar{3}$ rather than the original $\bar{0}$ or $\bar{1}$. 
% This will allow Bob to convey more information with just two codewords. 
such that Alice interprets $\bar{0}$ and $\bar{1}$ differently for the rest of the block depending on whether she first decoded a $\bar{0}$ or $\bar{1}$ within the block. The bits communicated in the rest of the block can now be combined with the first heard bit to take on more than two meanings. 
% of all four original codewords. Unfortunately, this doesn't quite work as an adversary 
% Ideally, the rest of the block can now be used to convey the original meaning of $\bar{0}$ and $\bar{1}$ if it started with $\bar{1}$, or $\bar{2}$ and $\bar{3}$ if it started with $\bar{1}$. This idea takes quite a bit of detail to actually implement correctly.

%Then, the original meanings of $\bar{0}$ and $\bar{1}$ can be conveyed by Bob starting a block by sending $\bar{1}$ and then using $\bar{0}$ and $\bar{1}$ as he originally did, while the original meanings of $\bar{2}$ and $\bar{3}$ can be conveyed by starting a block $\bar{0}$ and then using $\bar{0}$ and $\bar{1}$ in a new way. This turns out to introduce many other problems, unfortunately, so we have to do a lot more work to make this actually work.

To demonstrate the technique, let us show how to do incrementation. Incrementation will be done in such a way that a $\bar{1}$ is always heard first before any $\bar{0}$ within a block. This will leave hearing a $\bar{0}$ first within a block open to having a new meaning.

More specifically, a $\bar{1}$ at the beginning of a block indicates to Alice to increment her counter. Hearing a $\bar{0}$ after hearing a $\bar{1}$ within the same block indicates that Bob has noted her incrementation, and that she may increment again next block. Otherwise, if Alice's current value of $\cnt$ has not been confirmed by receiving a $\bar{0}$, she does nothing when she receives a $\bar{1}$ at the beginning of the next block. On Bob's end, as long as the value of $\cnt$ is less than the desired target $i$, he always begins a block by sending $\bar{1}$, and only switches to sending $\bar{0}$ when Alice informs him that she's seen a $\bar{1}$ this block (this requires Alice to send a new piece of information each message). In this way, Alice cannot over-increment without Bob's permission, so the incrementation can be done in sync.

Now, when Alice receives a $\bar{0}$ first within a block, she knows the incrementation is over. If only she knew which question (value of $x[\cnt]$ or parity of $\cnt$) Bob wants answered, we would be done! Unfortunately, we don't have any codewords left for Bob to send Alice to tell her this last bit of information. Luckily, we don't need another codeword -- we can simply reuse the counting technique! That is, to learn the question, Alice participates in a new incrementation of a \emph{second} counter. When this new incrementation is over, the final value of this second counter indicates which of the two questions Bob would like answered. Then, Alice can begin sending the answer bit for the rest of the protocol. 

There are many details that need to be ironed out to make this intuitive outline work. We do so in Section~\ref{sec:3/5}. 

==> old-intro.tex <==
\section{Introduction}

Consider the following task: Alice wishes to convey a message $x$ to Bob in a way such that even if a constant fraction of the communicated bits are adversarially tampered with, Bob is still guaranteed to be able to determine her message. Can she do this, and what is the largest number of adversarial errors their communication can be resilient to?

One widely studied approach to this problem is that of \emph{error correcting codes}. In an error correcting code, each possible message $x$ is associated with a longer codeword, such that the Hamming distance between any two codewords is a constant fraction of the length of the codewords. Then, to communicate a message $x$, Alice sends Bob the corresponding codeword. The point is that since the distance between any two codewords is large, an adversary must corrupt a large fraction of the communication in order for Bob to decode to the wrong codeword. 
% \mnote{i rly like this intro!! small thing -- we never mention that distance is calculated as smallest distance. idk if it's too obvious.}

By the Gilbert-Varshamov bound, the best possible relative distance\footnote{The relative distance of an error-correcting code is the maximum possible minimum distance between two codewords, as the number of codewords approaches $\infty$. In general, when we talk about relative distance or error resilience, we mean as the number of possible messages $x$ approaches $\infty$.} of any error correcting code over the binary alphabet is $\le \frac12$. Since the relative distance of an error correcting code is precisely its resilience to adversarial erasures, this means that to communicate $x$ to Bob over a binary channel, if Alie simply sends an error correcting code, she can be resilient to at most $\frac12$ adversarial erasures, but no more. Whether there exists a protocol with resilience to $> \frac12$ adversarial erasures was previously unknown. \mnote{Feel free to reword, but the general sentiment is that "simply sending an ECC" doesn't sound right.}

% Over large alphabets, there are known constructions of error correcting codes that achieve distance $\approx 1$. \mnote{i'm not actually sure it makes sense to mention large alphabet at all. weak opinion though. } Over the binary alphabet, however, the best possible distance of any error correcting code is $\le \frac12$, by the Gilbert-Varshamov bound.\mnote{we do need to get across here or somewhere else that we mean limit is 1/2 as Alice's input size gets large.} In the case of erasures, the distance of an error correcting code is precisely its resilience to adversarial erasures. 
% This means that to commuicate $x$ to Bob over a binary channel, if Alice simply sends an error correcting code, she can be resilient to at most $\frac12$ adversarial erasures, but no more.
% \mnote{Feel free to reword, but the general sentiment is that "simply sending an ECC" doesn't sound right.}
% Whether there exists a protocol with resilience to $> \frac12$ adversarial erasures was previously unknown.

In this work, we show that there is in fact a way for Alice to communicate $x$ to Bob such that Bob is guaranteed to learn $x$ \emph{even if more than half of the communicated bits are erased!} To do this, we introduce the notion of an \emph{interactive error correcting code ($\iECC$)}, which is an interactive protocol with a fixed length and speaking order, such that Bob can still correctly learn $x$ as long as not too large a fraction of the total communication was erased. Perhaps surprisingly, by leveraging the power of interaction, we design an $\iECC$ that is resilient to $\frac35$ adversarial erasures.

Note that a classical error correcting code is an $\iECC$ in which Alice speaks in every round. Our result essentially shows that Bob talking occasionally \emph{instead of Alice} actually improves the error resilience. It is not obvious that this should be the case -- since Bob can only send feedback, while Alice can actually send new information, Bob's messages a priori seem a lot less valuable than Alice's. How can the error resilience be improved when messages containing information about $x$ have been replaced by messages without? Nevertheless, we show that these feedback messages play a vital role in increasing the error resilience past $\frac12$. 

\subsection{Our Results.}

Our main result is an $\iECC$ that achieves an erasure resilience of $\frac35$. 

\begin{theorem}
    For any $\epsilon > 0$, there exists an $\iECC$ over the binary erasure channel resilient to $\frac35-\epsilon$ erasures, such that the communication complexity for inputs of size $n$ is $O_\epsilon(n^2)$.
\end{theorem}

We also prove the following lower bound.

\begin{theorem}
    There does not exist an $\iECC$ over the binary erasure channel resilient to $\frac23$ erasures.
\end{theorem}

Consider the problem of constructing an $\iECC$ over the binary \emph{bit flip} channel, as opposed to the binary erasure channel. In this setting, instead of erasing bits, an adversary may toggle bits of her choice. A standard (non-interactive) error correcting code can achieve a distance of $\frac12$, giving a trivial non-interactive $\iECC$ resilient to $\frac14$ adversarial bit flips.

We prove the following negative result on the maximal possible error resilience to bit flips of any $\iECC$ scheme.

\begin{theorem}
    There does not exist an $\iECC$ over the binary bit flip channel resilient to $\frac27$ adversarial bit flips.
\end{theorem}

We do not know of any constructions of $\iECC$s that achieve a higher error resilience to bit flips than the standard (non-interactive) error correcting code. We leave open the problem of constructing such an $\iECC$.

\subsection{Related Work}

A long line of works starting with \cite{Schulman92,Schulman93,Schulman96} and continuing with \cite{BravermanR11,Braverman12,BravermanE14,GellesHKRW16,BrakerskiK12,BrakerskiN13,GellesHKRW16, GellesH17,EfremenkoGH16,GhaffariHS14,EfremenkoKS20b} studies the problem of constructing error resilient interactive protocols, albeit for two-way communication. 

% \cite{GellesHKRW16} (channel capacity for adversarial bit flips)
% \cite{GellesH17} (channel capacity for feedback and erasures)

There are two sub-lines of work most relevant to our work:
\begin{itemize}
    \item {\bf List-Decoding to Unique-Decoding.} List-decoding \cite{Elias57,Wozencraft58} is a protocol for one-way communication at the end of which the receiver obtains a small list of values, of which the sender's value must be one. The work of \cite{GhaffariHS14} showed how to go from list-decoding (to polylog values) to unique decoding to construct an error-resilient scheme for two-way communication. The later work of \cite{EfremenkoKS20b} applied this technique to the binary alphabet setting, and for a list-decoding scheme with list of size 3. \mnote{I'm still not sure I agree a ton with the premise that this is super important for our work, even if it's where the idea came from. I'd rather focus on basic IC results, e.g. asserting that 2-way is 1/4 error resilient for bit flip)
    \item {\bf Schemes Over Binary Erasure Channels.} The works of \cite{GellesH17,EfremenkoGH16,KalaiGZ21a} construct interactive protocols for two-way communication over a binary channel resilient to a constant fraction of adversarial erasures. The work of \cite{GellesH17} constructed such a scheme with minimal asymptotic rate. The problem of the maximal erasure resilience was first studied by \cite{EfremenkoGH16} and was fully solved by \cite{KalaiGZ21a}.
\end{itemize}

% As mentioned earlier, an interactive error correcting code can be thought of as a nonadaptive interactive protocol where Alice wants to communicate $x$ to Bob, but Bob does not need to communicate anything to Alice. This one-way setting has never been studied before, but the two-way setting has many prior results. In the usual setting, Alice and Bob each have a private input, $x$ and $y$ respectively, and there is a noiseless protocol $\pi_0$ of length $|\pi_0|$ that computes $f(x,y)$. The goal is to design a protocol $\pi$ that also computes $f(x,y)$, has length $c|\pi_0|$, and is resilient to adversarial errors. This is studied over both the binary bit flip and erasure channels, and also over both the large alphabet bit flip and erasure channels. The goal is usually to maximize the error resilience of the protocol (the fraction of adversarial errors it is resilient to).

% The work of \cite{KalaiGZ21a} resolves this question fully for the erasure channel of all input sizes, and finds that the best possible error resilience is always $\frac12-\epsilon$. This problem was originally posed and studied in \cite{EfremenkoGH16}.

% Study of the bit flip channel is more complicated. explain...

% For a full survey of the history of coding for interactive communication, refer to \mnote{cite survey}.

% Usually, in this two-way interactive setting, interaction is considered a burden. The protocol must be reslient to the adversary choosing to corrupt either Alice or Bob, rather than in the classical setting where the adversary can only corrupt the sender. However, our work is different because it presents interaction as a tool rather than a burden.

% \paragraph{Related Work in List Decoding.}

% list-decoding: \cite{Elias57,Wozencraft58} \cite{BravermanE17}

% \cite{GhaffariHS14} -- list decoding to unique decoding
% \cite{EfremenkoKS20b} -- 5/39

\subsection{Technical Overview}

\subsubsection{A Simpler $6/11$ $\iECC$}

We begin by discussing a simpler scheme that achieves an erasure resilience of $\frac6{11}$. Our starting point is the list-decoding to unique-decoding paradigm of \cite{GhaffariHS14,EfremenkoKS20b}:
\begin{enumerate}
    \item Alice and Bob engage in a list-decoding scheme such that Bob ends up with a small list of values, with the guarantee that Bob's list contains Alice's input assuming there were not too many corruptions. 
    \item Bob sends the small list to Alice, encoded in an error correcting code.
    \item Alice decodes Bob's message to obtain a small list. She replies with an error correcting encoding of the index of her input in the list.
\end{enumerate}
% Assuming that the total number of corruptions is not too high, correctness can be argued by noting that Bob's list must contain Alice's input, Alice receives Bob's list correctly, and that the set of all Alice's messages cannot have been corrupted too much. 
% \cite{EfremenkoKS20b} uses this paradigm to construct an interactive protocol for two-way communication in the binary bit-flip setting whose error resilience beats the trivial resilience of $\frac18$ (obtained by Alice and Bob each sending an error correcting encoding, with distance $\frac12$, of their own input). To do this, they leverage two facts: (1) There exists a list-decoding scheme whose correctness property holds for higher error rates than in the unique-decoding setting. (2) If the resulting list is of small constant size, say 3, there exists a set of 3 codewords (e.g. $(001)^M, (010)^M, (100)^M$) that Alice may send at the end that has distance greater than the asymptotic $\frac12$ upper bound for error correcting codes. Combining these two error resilience inflations, they obtain a protocol that is resilient to $> \frac14$ corruptions to Alice's messages.
% These two properties carry over to our setting, the binary erasure channel, as well:
Over a binary erasure channel, the first and third steps and can be implemented in the following manners:
\begin{enumerate}
    \item Since the adversary can only erase and cannot toggle bits, this means that the original message must contain the bits that are received. Suppose Alice sends $\ECC(x)$, where $\ECC$ is an error correcting code of distance $\frac12$. Then, it can be shown that as long as less than $\frac34$ of the bits are erased, there are at most two codewords compatible with the received bits! This gives us a list-decoding scheme where the resulting list is of size $2$ that is resilient to $\frac34$ erasures.
    \stepcounter{enumi}
    \item Assuming that Alice decodes Bob's list of size 2 correctly, she can simply send $0^M$ or $1^M$ to indicate to Bob which of the two inputs were hers.
\end{enumerate}
Since Alice's final message has relative distance $1 > \frac12$, this increases the distance between Alice's messages for any two distinct inputs and gives a one-way protocol resilient to $> \frac12$ erasures to Alice's messages.

However, this does not constitute a protocol for one-way communication resilient to $> \frac12$ erasures to the \emph{total} communication! It turns out that in order for Alice to correctly learn Bob's list, Bob's messages must take up a significant portion of the total communication, so that $> \frac12$ of Alice's messages is less than $\frac12$ of the total communication. So it appears we have not yet made progress past the $\frac12$ erasure resilience attained by error-correcting codes.

The issue was that as Bob sends $\ECC(L)$, where $L$ is the list of size $2$, an adversary can simply erase half of Bob's message so that Alice cannot tell whether Bob's list were $L$ or $L'$. Then Alice cannot know whether to tell Bob that she has the first or second item in the list. This attack requires only half of Alice's first message, followed by half of Bob's message, for a total of less than half of the total communication.

We solve this problem as follows: Instead of having Bob send a list $L = \{ x_0, x_1 \}$ to Alice via an error correcting code, he communicates an \emph{index} $i$ for which $x_0[i] \not= x_1[i]$ via a \emph{counting technique}. In this counting technique, the protocol is divided into many \emph{chunks} in which Alice sends a fixed-length message, then Bob sends a fixed-length message. Alice keeps track of a counter $\cnt$ initially set to $0$ and sends $\cnt$ along with her input $x$ to Bob in each chunk (encoded with an error correcting code). Bob's goal is to tell Alice to increment her counter until it reaches $i$, and then to send him the bit $x[i]$ for the rest of the protocol so that he can distinguish $x_0$ from $x_1$. The goal is to do this with as few possible distinct message contents from Bob as possible (note that if Bob sends a super-constant number of possible codewords each chunk, then the distance between the codewords asymptotically approaches $\frac12$, and the adversary can once again employ the attack where she erases half of Alice's messages and half of Bob's).

As a first attempt, Bob might send a codeword $\bar{1}$ to indicate to Alice that she should increment her counter, and $\bar{0}$ to indicate that she should stop. Then, Alice will increment her counter once each chunk until she receives $\bar{0}$, at which point she begins sending $x[\cnt]$. The problem here is that the adversary can simply erase all of Bob's message in chunk $i$, so that Alice increments her counter too far! Alternatively, Alice could only increment her counter when she receives $\bar{1}$, but now the adversary can erase Alice's message so that Bob can't tell if Alice has reached $i$ or has passed it.

Instead, Alice increments her counter only when she sees that Bob's message has changed from $\bar{0}$ to $\bar{1}$, or vice versa. Bob will then wait until he sees that her counter has been incremented correctly before flipping his message to get Alice to increment her counter again. This way, Alice and Bob can make sure they're on the same page with the value of the counter: Bob only indicates to Alice that she should increment again when he notes her previous incrementation.

When Bob sees that Alice's counter has reached the index $i$, he begins sending a third codeword $\bar{2}$ to ask Alice for the value of her input at index $i$. Once Bob has begun sending $\bar{2}$'s, note that Alice will never increment her counter again, since she only increments when she unambiguously receives a $\bar{0}$ or $\bar{1}$ from Bob. Thus, as long as Alice unambiguously receives $\bar{2}$ at some point, she will have correctly learned $i$ and begins sending the value of $x[i]$.

Recall, however, that Bob can see two possible values of $x$, which means that he can also see two different counter values associated with each value of $x$. If the counters increment simultaneously (meaning that Bob never list-decodes to $(x_0, \cnt_0)$ and $(x_1, \cnt_1)$ with $\cnt_0 \not= \cnt_1$), then the above techniques work and are sufficient for Alice to learn the index $i$ correctly.

If the counters ever get out of sync, however, note that they must be off by $1$ (if the first time the counters get out of sync one is at least $2$ greater than the other, then Bob can conclude that one made an impossible increment and thus deduce $x$). In this case, Bob can begin sending a fourth codeword $\bar{3}$, asking Alice to tell him the parity of her counter. Once again, note that this halts the counting process, as Alice will never again unambiguously decode $\bar{0}$ or $\bar{1}$.

In total, Bob uses four total codewords throughout the entire protocol. These can have distance $\frac23$: for instance, the codewords $(000)^M, (110)^M, (101)^m, (011)^M$. By letting Alice's messages have length $\frac83 M$ and the number of chunks be sufficiently large, any adversary strategy for confounding Bob must, in nearly every chunk, either corrupt $\frac34$ of Alice's message, or $\frac23$ of Bob's message and $\frac12$ of Alice's (otherwise Bob can uniquely decode Alice's message to learn $x$). This means that the protocol is resilient to 
\[
    \frac{\frac34 \cdot \frac83 M }{\frac83 M + M} = \frac{\frac23 M + \frac12 \cdot \frac83 M}{\frac83 M + M} = \frac6{11}
\]
erasures.

For a more formal statement and analysis of this $6/11$ protocol, we refer the reader to Section~\ref{sec:6/11}.


\subsubsection{Improving $6/11$ to $3/5$}

In the above protocol, Bob uses two different codewords to increment Alice's counter. Then, when he wants to ask Alice for either the value of $x[\cnt]$ or the parity of $\cnt$, he has to use two \emph{new} codewords to convey the appropriate question. If we were able to somehow ask this question without the use of these two new codewords, the relative distance between Bob's codewords could increase to $1$. Then, by letting Alice and Bob speak into a $4:1$ ratio, an adversary would have to corrupt either $\frac34$ of Alice's message or all of Bob's and $\frac12$ of Alice's. This increases the erasure resilience to
\[
    \frac{\frac34 \cdot 4M}{4M + M} = \frac{M + \frac12 \cdot 4M}{4M + M} = \frac35.
\]

To encapsulate the meanings of $\bar{2}$ and $\bar{3}$ with just two codewords $\bar{0} = 0^M$ and $\bar{1} = 1^M$, the main idea is to have $\bar{0}$ and $\bar{1}$ mean different things at different points in the protocol. Let us divide the protocol into \emph{blocks} of chunks, such that it means something different whether Alice first hears a $\bar{0}$ or $\bar{1}$ within each block. This will allow Bob to convey more information with just two codewords. 

To demonstrate the technique, let us show how to do incrementation. Incrementation will be done in such a way that a $\bar{1}$ is always heard first before any $\bar{0}$ within a block. This will leave hearing a $\bar{0}$ first within a block open to having a new meaning.

More specifically, a $\bar{1}$ at the beginning of a block indicates to Alice to increment her counter. Hearing a $\bar{0}$ after hearing a $\bar{1}$ within the same block indicates that Bob has noted her incrementation, and that she may increment again next block. Otherwise, if Alice's current value of $\cnt$ has not been confirmed by receiving a $\bar{0}$, she does nothing when she receives a $\bar{1}$ at the beginning of the next block. On Bob's end, as long as the value of $\cnt$ is less than the desired target $i$, he always begins a block by sending $\bar{1}$, and only switches to sending $\bar{0}$ when Alice informs him that she's seen a $\bar{1}$ this block (this requires Alice to send a new piece of information each message). In this way, Alice cannot over-increment without Bob's permission, so the incrementation can be done in sync.

Now, when Alice receives a $\bar{0}$ first within a block, she knows the incrementation is over. If only she knew which question (value of $x[\cnt]$ or parity of $\cnt$) Bob wants answered, we would be done! To learn the question, Alice participates in a new incrementation of a \emph{second} counter. When this new incrementation is over, the final value of this second counter indicates which of the two questions Bob would like answered. Then, Alice can begin sending the answer bit for the rest of the protocol. 

There are many details that need to be ironed out to make this intuitive outline work. We do so in Section~\ref{sec:3/5}. 

\subsubsection{Lower Bounds}

We also prove lower bounds on the maximal possible error resilience of any $\iECC$. In particular, we prove lower bounds of $\frac23$ in the binary erasure setting and $\frac27$ in the binary bit flip setting. These are proved in Sections~\ref{sec:2/3} and~\ref{sec:2/7} respectively.




% Recall that an interactive error correcting code, or an $\iECC$, is a nonadaptive interactive protocol between Alice and Bob where Alice holds $x\in\{0,1\}^n$ and Bob must output $x$ at the end of the protocol. The $\iECC$ is considered $\epsilon$-error resilient in the binary erasure channel if Bob will output the correct value of $x$ even with an adversary erasing $\epsilon$-fraction of the total communication. As $n$ gets large, a classical $\ECC$ can achieve $\frac12$ error resilience, but no better.

% Before we present our $\frac35$-error resilient protocol, we present a simpler protocol that is resilient to $\frac6{11}$ error. This will use the same core technique as the final $\frac35$ protocol.

% Recall that we need to fix which of Alice and Bob speaks in each round beforehand. Our protocol will consist of many equal-length \emph{chunks}, each consisting of a fixed number of rounds from Alice to Bob followed by a different fixed number of rounds from Bob to Alice. We say that all the rounds spoken by a single party within a chunk is a \emph{message}. 

% Our protocol will use a function $\ECC(x)$, which denotes a classical error correcting code that is $\frac12$-error resilient, and also has some other natural properties.

% At a high level, our protocol works as follows:
% \begin{enumerate}
%     \item 
%         The protocol begins with Alice sending $\ECC(x)$ to Bob as her message in each chunk. If the adversary ever erases $<\frac12$ of Alice's message, Bob will learn $x$. However, the protcol should be resilient to $>\frac12$ error, so this isn't enough. Instead, we will use the fact that if the adversary ever erases $<\frac34$ of Alice's message, Bob can narrow $x$ down to two possibilities. As long as Alice speaks $<\frac8{11}$ in each chunk, this is guaranteed to happen at some point.
%     \item \label{item:i}
%         Let Bob's two possilities for $x$ be $x_0$ and $x_1$. At this point, Bob will send Alice $i$, an index on which $x_0$ and $x_1$ differ.
%     \item 
%         When Alice receives Bob's query for index $i$, she begins sending only the bit $x[i]$ in every subsequent round (so that messages consist of a string of all $0$s or all $1$s). Now, as long as Bob hears any one bit from Alice, he learns $x[i]$, and therefore $x$. The advantage is now Alice possible messages are distance $1$ apart instead of distance $\frac12$, so Bob only needs to hear one of her bits, rather than $\frac12$ of her bits to uniquely decode her message.
% \end{enumerate}

% It remains to describe how Bob communicates an index $i$ to Alice. Note that simply sending $\ECC(i)$ in each message will not work: a chunk with $<\frac6{11}$ error only guarantees that Alice hears $>\frac13$ of Bob's message, not $\frac12$, which is what is needed to uniquely determine $i$ from an error correcting code. (In the case where Bob instead hears $>\frac12$ of Alice's message, he can uniquely determine $x$, which would also make the protocol successful.) 

% Instead, we use a counting technique: Alice keeps track of a counter initially set to $0$ and sends $x$ along with $\cnt$ to Bob each message (encoded in an $\ECC$).



% The protocol is described formally in Protocol~\ref{prot:6/11}.

==> old/2.3-upper-bound.tex <==
\subsection{Binary Erasure Channels} \label{sec:2/3}

\begin{theorem}
    No interactive binary protocol for one way communication is resilient to a $\frac23$ fraction of erasures with probability greater than $\frac12$.
\end{theorem}

\begin{proof}
    Consider the frequency with which Bob speaks. If he speaks $r \le \frac13$ of the time, consider the following attack: the adversary erases all of Bob's messages. Then, Alice's messages to Bob reduce to the case of an error correcting code, which has distance at most $\frac12$. Thus, the adversary can corrupt half of Alice's messages such that Bob can distinguish between two of Alice's inputs. This gives a corruption rate of $r + \frac{1-r}{2} = \frac{1+r}{2} \le \frac23$.
    
    Alternatively, if Bob speaks $r > \frac13$ of the time, the adversary can simply erase all of Alice's messages to Bob. Then, Bob receives no information about Alice's input. This attack requires $< \frac23$ corruptions. 
    
    Thus, there is always an attack using $\le \frac23$ corruptions for which Bob cannot correctly output Alice's input with probability greater than $\frac12$. 
\end{proof}

==> old/4.7-construction.tex <==
\subsection{One-Way Interactive Protocol Resilient to $4/7$ Erasures} \label{sec:4/7}

\protocol{Interactive Binary One Way Protocol Resilient to $\frac4{7} - \epsilon$ Erasures}{4/7}{
    Let $n$ be the size of the message $x \in \{ 0, 1 \}^n$ that Alice wishes to convey to Bob. Let $\bar{0}, \bar{1}, \bar{2}$ denote length $6M$ binary strings that have relative distance $\frac23$ from each other (for instance, $(100)^{2M}, (010)^{2M}, (001)^{2M}$ are such strings). Let $\ECC(\cdot, \cdot, \cdot, \cdot) : \{ 0, 1 \}^n \times [0,n] \times \{\true, \false \} \times \{ \true, \false \} \rightarrow \{ 0, 1 \}^{6M}$ be an error correcting code of relative distance $\frac12-\epsilon$ such that each codeword is also relative distance $\ge \frac12 - \epsilon$ from each of $\bar{0}, \bar{1}, \bar{2}$. Our protocol consists of $B = \frac{10n}{\epsilon}$ blocks of $T = \frac{10}{\epsilon}$ chunks of $7M$ rounds, composed of Bob sending a $M$ bit message followed by Alice sending an $6M$ bit message.
    
    \begin{itemize}
    \item {\bf Alice:} 
        In addition to $x$, Alice holds:
        \begin{itemize}
            \item a counter $c$ taking values in $[0, n]$, initially set to $0$,
            \item a bit $s\in \{\true,\false\}$ (sent) denoting whether she has received a $0$ from Bob after sending this particular value of $c$ (i.e. whether she has received confirmation that $c$ was successfully sent to Bob); initially $s$ is set to $\true$,
            \item a bit $t\in \{\true,\false\}$ (toggle) denoting whether she has received a $1$ so far this block; $t$ is initially set to $\false$.
        \end{itemize}
        
        At the beginning of each block, she resets $t = \false$. She begins the block by sending $\ECC(x, c, s, t) \in \{ 0, 1 \}^{6M}$ in each chunk. If in a chunk she receives a $1$ from Bob, she sets $t \gets \true$ and, if $s = \true$, increments $c$ and sets $s \gets false$. If she ever receives a $0$ she does the following:
        \begin{itemize}
            \item If $t=\true$ (i.e. she's already seen a $1$ this block), she sets $s\leftarrow \true$.
            \item If $t=\false$, she forgoes all future instructions and in all future chunks sends the same codeword in $\{ \bar{0}, \bar{1}, \bar{2} \}$, as follows: if $c$ is even, she sends $x[c/2]$, and if $c$ is odd, she sends $\bar{2}$.
        \end{itemize}
        
    \item {\bf Bob:} Bob ignores all chunks where at least $\frac34-\epsilon$ of the input has been erased. In all other chunks, he can narrow down Alice's message to two options: $(x_1,c_1,s_1,t_1)$ and $(x_2,c_2,s_2,t_2)$. $x_1$ and $x_2$ must be consistent throughout the protocol, or Bob can know the one that changed was a lie. $c_1$ and $c_2$ must increment by 0 or 1 each time, or Bob knows the corresponding world is fake.
    
    Start each block sending 1's. In a chunk, if Bob doesn't receive at least $\frac34-\epsilon$ messages, he just sends the same message as the previous. However, if Bob receives a message where $t_1=t_2=\true, c_1=c_2$, send 0's for the rest of the block. 
    
    If $c_1\neq c_2$ or $c_1=c_2$ and $c/2$ is an index where the two value $x_1$ and $x_2$ differ, send 0 forever.
    
    Else if $t_1\neq t_2$ (wlog $t_1=\false$), send 0 for the rest of the block, and start the next block with 1's as you usually would, with the following extra caveat. If the first message you receive from Alice no longer has something that decodes to $(x_1,c_1,s_1,t_1)$, abort everything you're doing, and just try to increment $c_2$ so that it's the opposite parity of the last value of $c_1$ you saw. Otherwise, resume as normal.
    
    At the end, decode the last message you received from Bob where you got at least $\frac13+\epsilon$ bits. You can uniquely figure out $d\in \{\bar{0}, \bar{1}, \bar{2}\}$. If the last time you received $(x_1,c_1)$, this pair corresponds to $d$, answer $x_1$, else answer $x_2$.
    \end{itemize}
}

\begin{lemma}
    There are $n+5$ blocks with error $<\frac47-10\epsilon$. In any such block, there are $10$ chunks with error $<\frac47-\epsilon$.
\end{lemma}

\begin{proof}
    
\end{proof}

\begin{theorem}
    The protocol given in Figure~\ref{prot:4/7} is resilient to a $\frac4{7}-100\epsilon$ fraction of erasures.
\end{theorem}

\begin{proof}
    We show that as long as the adversary corrupted at most $\frac4{7} - 100\epsilon$ of the rounds, Bob successfully outputs Alice's input $x$. To this end, suppose for the sake of contradiction that the adversary can corrupt $\le \frac4{7} - 100\epsilon$ of the rounds such that Bob outputs the incorrect value of $x$. First, we may assume that none of the shortcuts described in the protocol happen: the adversary corrupts at least $\frac12-\epsilon$ of each of Alice's message (at least, up until she successfully receives a 0 at the start of a block), the indices $c_0$ and $c_1$ begin at $0$ and increment, the values of $x_0$ and $x_1$ remain the same in every of Alice's messages that have been corrupted less than $\frac34-\frac32\epsilon$, etc. 
    
    Let $R+1$ be the first block in which Alice hears 0 at the beginning of a block. (if this never happens, let $R = T$). Then, for blocks before or equal to $R$, Alice always sent $\ECC(x, c, ?, ?)$, and in all future blocks, Alice always sends something in $\{\bar{0}, \bar{1}, \bar{2}\}$. If Bob receives at least $\frac13$ bits in any chunk after block $R$, he will correctly deduce $x$. The counters are guaranteed to have not changed from the last time Bob heard them, since if he ever planned on sending 0's when Alice could possibly hear at the start of the block, he only sent 0's in the previous block since the last time he heard Alice's message, and hearing 0's can never increment Alice's counter. The mapping $(x,c)\to \{\bar{0}, \bar{1}, \bar{2}\}$ is guaranteed to be injective, based on Bob's condition of moving to this phase. 
    
    Thus, to fail, it has to be the case that none of Alice's messages after block $R$ got through to Bob.
    
    We assumed that in each of the first $R$ blocks, at least half of Alice's bits to Bob are corrupted, otherwise Bob can correctly learn $x$. Let $S$ be the number of of these $R$ blocks in which at most $\frac47-10\epsilon$ messages are corrupted. In each of these, there are at least 10 chunks where Alice and Bob both hear each other. Whenever this happens, in the chunk one of the two possible counters that Bob has either advances, or becomes confirmed (that is, $s=\true$), or moves to the new phase (sending $\bar{0}, \bar{1}, \bar{2}$). There are only $4(n+5)+1$ such advances that could possibly occur, without Alice actually advancing to the next stage, or the counters diverging. Thus, the protocol must advance to the stage where Alice sends $\bar{0}, \bar{1}, \bar{2}$.
\end{proof}




==> upper-bounds/graph.tex <==
\subsection{Potential Graph Upper Bound}

\rnote{for if we want to write up the graph upper bound}

==> x-two-way-erasure.tex <==
\section{Two Way Binary Erasure Channels}



\subsection{$1/2$ Efficient Construction}

\begin{figure}[h!]
    \centering
    \protocol{}{
        Let $\pi$ be an error-free binary protocol that runs in $n_0$ rounds. We may assume that $\pi$ is alternating (i.e. Alice and Bob take turns speaking) with at most a factor of $2$ blowup in the round complexity. We simulate $\pi$ with an erasure-resilient protocol that occurs in $N = \frac{9 n_0}{2\epsilon^2}$ rounds, with Alice and Bob taking turns speaking. These rounds are partitioned into $\frac{3n_0}{2\epsilon}$ blocks of $\frac{3}{\epsilon}$ rounds. Assume that $\frac{3}{\epsilon}$ is an even integer, so that Alice speaks first within each block. Let $c : 1 \mapsto 11, 0 \mapsto 10$ be an encoding of the bits $\{ 0, 1 \}$. 
        
        \vspace{0.075in}
        
        Alice and Bob each have an internal mode, which is either $\speaker$, $\listener$, or $\passer$. They also track an internal transcript equal to what they believe the current noiseless protocol is (initially it is $\emptyset$). Their behavior is described as follows:
        \begin{itemize}
            \item A party in $\listener$ mode sends a $1$ whenever they receive a message, and a $0$ when they don't. (Since Alice speaks first in a block and Bob did not send the previous message, she sends a $0$ for the first message in the block.) If a party begins a block in $\listener$ mode and the first non-erased message they receive is a $0$, they switch immediately to being in $\speaker$ mode. They also note the sequence of bits received in the previous block where at least one bit was received, and decode this to $m = 0$ or $m = 1$ based on whether at least one $0$ was heard after at least one $1$ was heard. Then, they add $m$ to their internal simulated transcript.
            \item When a party is in $\speaker$ mode and wants to communicate $m \in \{ 0, 1 \}$, they send the first bit of $c(m)$ repeatedly until they receive a $1$, then they send the second bit of $c(m)$ until they receive a $1$, and then they send $1$'s for the rest of the block. If a confirmation bit (i.e. a $1$) was received for both bits of $c(m)$, they switch to being in $\passer$ mode at the beginning of the next block and append $m$ to their internal simulated transcript. Otherwise, they are still in $\speaker$ mode and begin the next block by trying to send $c(m)$ from scratch.
            \item A party in $\passer$ mode sends $0$'s until they receive a $1$, at which point they switch to being in $\listener$ mode and begin sending a $1$ whenever they receive a message (including the most recently received $1$) and a $0$ otherwise. 
        \end{itemize}
        
        Our protocol begins with Alice in $\speaker$ mode and Bob in $\listener$ mode. Each time a party is in $\speaker$ mode, they send the next message $m \in \{ 0, 1 \}$ in their internal simulated transcript.
        %Each time a party is in $\speaker$ mode, they try to communicate the next unsent message of $\pi$. It can be shown (Claim~\ref{claim:speaker}) that a party in $\speaker$ mode only switches to $\passer$ mode once it can be proved that the message of $\pi$ has been received successfully, so that a party that has entered $\speaker$ mode for the $k$'th time knows to communicate their $k$'th message in $\pi$.
    }
    \caption{Protocol Resilient to $\frac12 - \epsilon$ Erasures}
    \label{fig:erasure-1/2}
\end{figure}

Our protocol resilient to a fraction of $\frac12 - \epsilon$ erasures is given in Figure~\ref{fig:erasure-1/2}. For clarity, we describe the first few rounds of the protocol.
\begin{enumerate}
    \item 

        Alice begins the protocol in $\speaker$ mode with her first bit as the noiseless transcipt, and Bob begins the protocol in $\listener$ mode with an empty transcript. Alice tries to communicate the first message $\pi_1 \in \{ 0, 1 \}$ of $\pi$ to Bob by sending over the bits of $c(\pi_1)$ to Bob, \ynote{need to define $c$ since the reader will read this before reading the formal description} repeating a bit until she receives a $1$ from him. She then sends $1$'s for the rest of the block. If she received confirmation bits from Bob for the entirety of $c(\pi_1)$, she switches to $\passer$ mode at the end of block $1$. Note that Bob remains in $\listener$ mode for the duration of block $1$, since the first message he receives from Alice must be a $1$.  \ynote{Again, this last sentence is not self contained.}
        
    \item 
        If Alice did not receive both confirmation bits from Bob, she is still in $\speaker$ mode at the beginning of block $2$. The parties rerun block $1$, with Alice trying to communicate $\pi_1$ from scratch.
        
        If Alice did receive both confirmation bits from Bob, she is now in $\passer$ mode at the beginning of block $2$. She sends $0$'s until she receives a $1$, at which point she switches to $\listener$ mode, sending a $1$ everytime she receives a message (including the recently received $1$) and a $0$ otherwise. Bob begins the block in $\listener$ mode: then, as the first message he receives from Alice in the block is a $0$, he switches to $\speaker$ mode and tries to communicate $\pi_2$ to Alice (beginning with sending a $1$, which is the first bit of $c(\pi_2)$, immediately after the most recently received $0$). Note that if Alice does not receive any of Bob's $1$'s for some rounds, she continues to send $0$ by default (as she is still in $\passer$ mode), which coincides with her behavior if she were in $\listener$ mode. Eventually, if/when Alice receives a $1$, she switches to being in $\listener$ mode, and for the rest of the block Bob is the $\speaker$ trying to communicate $\pi_2$ to Alice. We point out that here, the roles of $\speaker$ and $\listener$ have been reversed.
    \item 
        Round $3$ can start with Alice and Bob in any of the following pairs of roles: $(\speaker, \listener)$, $(\passer, \listener)$, $(\passer, \speaker)$, $(\listener, \speaker)$. We've already described the interactions in the $(\speaker, \listener)$ and $(\passer, \listener)$ scenarios ($(\listener, \speaker)$ works symmetrically), so it remains to describe the $(\passer, \speaker)$ scenario. In this case, Alice sends $0$'s until she receives a $1$. Meanwhile, Bob sends $1$'s (since a $1$ is the first bit of $c(\pi_2)$) until he receives a $1$. We've already pointed out that Alice's behavior as $\passer$ and with Bob as $\speaker$ is equivalent to if she were in the $\listener$ role. Furthermore, Alice becomes $\listener$ as soon as she hears a $1$, so Bob cannot move onto the next bit of $c(\pi_2)$ before Alice becomes a listener. From this point on, their behavior is the same as in the $(\listener, \speaker)$ scenario.
    \item 
        In general, in block $j$, Alice and Bob can be in any two different roles (Claim~\ref{claim:modes}), with behavior as described above.
\end{enumerate}

\begin{claim} \label{claim:modes}
    Alice and Bob can never be in the same mode at the same time.
\end{claim}

\begin{proof}
    First, they begin in different modes ($\speaker$ and $\listener$). We show that if they are in two different modes at the beginning of a block, then they cannot end up in the same mode during that block.
    
    If Alice and Bob are $\speaker$ and $\listener$ in some order at the beginning of a block, the $\speaker$ can become a $\passer$ at the end of the block, but the $\listener$ cannot become a $\speaker$ within that block: otherwise, the $\listener$ must've heard a $0$ initially from the $\speaker$, which is impossible. Otherwise, if Alice and Bob are $\passer$ and $\listener$ in some order, the $\passer$ can only become a $\listener$ once they receive a $1$, which happens only after the $\listener$ has received a $0$ and become a $\speaker$. From there, the $\listener$ cannot transition during the block since they did not start as a $\listener$ at the beginning of the block. The $\speaker$ also doesn't transition until the end of the block at earliest. Finally, if Alice and Bob are $\passer$ and $\speaker$ in some order, the $\speaker$ cannot become a $\passer$ until the other party has confirmed both bits of $c(m)$, at which point they must be a $\listener$.
\end{proof}

\begin{claim} \label{claim:speaker}
    When a party in $\speaker$ mode aiming to communicate message $m$ leaves $\speaker$ mode, the other party must've received $c(m)$. 
\end{claim}

\begin{proof}
    Recall that a $\speaker$ only transitions to $\passer$ mode once they've received confirmation bits for both bits of $c(m)$. Recall that the other party must be in either $\passer$ or $\listener$ mode during this process, and thus only sends $1$ if they received the $\speaker$'s message (which must be correct). Thus, the other party has received both bits of $c(m)$.
\end{proof}

\begin{theorem}
    The protocol in Figure~\ref{fig:erasure-1/2} is resilient to a $\frac12 - \epsilon$ fraction of erasures.
\end{theorem}

\begin{proof}

    We begin with the following claim.
    
    \begin{claim}
        We first claim that if a block has at most $\frac12 \cdot \frac3\epsilon - 3$ corruptions, then the next unsent message of $\pi$ is successfully received and the $\speaker$ switches to being in $\passer$ mode. 
    \end{claim}
    \todo{change statement of lemma to match the proof}

    \begin{proof}
        To show this, we consider the possible combinations of Alice and Bob's starting modes.
        
        If Alice and Bob are in $\speaker$ and $\listener$ mode, respectively, there are at least $3$ pairs of consecutive Alice-Bob rounds for which neither message is erased. Then, in the first such pair, Alice is able to send the first bit of $c(\pi_i)$ and receive confirmation from Bob, and in the second such pair, she sends the second bit of $c(\pi_i)$ and receives confirmation. She then switches to $\passer$ mode at the end of the block. The case where Alice is $\listener$ and Bob is $\speaker$ is identical, except we disregard Alice's first and last rounds and consider Bob-Alice pairs of messages. There are at least $2$ non-erased pairs, which is enough for Bob to communicate $c(\pi_i)$ and receive confirmation bits.
        
        If Alice and Bob are in $\passer$ and $\listener$ mode, respectively, then there is some first message where Alice's $0$ to Bob is not erased. Say that it is Alice's $j$'th message in the block. There must've been at least $j-1$ erasures prior to that point. After that point, consider Bob-Alice pairs of consecutive rounds, disregarding Alice's final round. There are $\frac12 \cdot \frac3\epsilon - j$ such pairs, so at least $2$ such pairs have no erasures. In these two pairs, Bob is $\speaker$ and conveys successfully $c(\pi_i)$ to Alice and receives her confirmation. He then switches to $\passer$ mode. The case where Bob is $\passer$ and Alice is in $\listener$ mode works analogously.
        
        The final case is where Alice and Bob are in $\passer$ and $\speaker$ mode, respectively. In this case, consider the first message from Bob to Alice that is not erased. Say that it is Bob's $j$'th message. Then the previous $j-1$ Bob's messages must've been erased. After this message, Alice is in $\listener$ mode. Consider Alice-Bob pairs of rounds after Bob's $j$'th message. At least $2$ of these pairs of rounds must be uncorrupted, which means that by the end of the block Bob will have sent $c(\pi_i)$ and received confirmation. The case where Alice is $\speaker$ and Bob is $\passer$ is analogous. 
    \end{proof}
    Now, it suffices to show that if there is a $\le \frac12 - \epsilon$ fraction of erasures, there must be at least $n_0$ blocks with at most $\frac12 \cdot \frac3\epsilon - 3$ corruptions. Let $\hat{n}$ denote the number of such blocks. Then, 
    \begin{align*}
        \hat{n} \cdot 0 &+ \left( \frac{3n_0}{2\epsilon} - \hat{n} \right) \cdot \left( \frac12 \cdot \frac3\epsilon - 2 \right) \le \left( \frac12 - \epsilon \right) \cdot \frac{9n_0}{2\epsilon^2} \\
        &\implies \frac{3n_0}{2\epsilon} \le \left( \frac12 \cdot \frac3\epsilon - 2 \right) \cdot \hat{n} < \frac12 \cdot \frac3\epsilon \hat{n} \\
        &\implies n_0 < \hat{n}.
    \end{align*}
    This means that in at least $n_0$ blocks, the next message of $\pi$ was successfully communicated, so that the entirety of $\pi$ is transmitted successfully.
    \todo{I think we should make it more rigorous that false messages can never be transmitted}
    
\end{proof}


